Transforming RDF-star to Property Graphs: A Preliminary Analysis of Transformation Approaches -- extended version

RDF and property graph models have many similarities, such as using basic graph concepts like nodes and edges. However, such models differ in their modeling approach, expressivity, serialization, and the nature of applications. RDF is the de-facto standard model for knowledge graphs on the Semantic Web and supported by a rich ecosystem for inference and processing. The property graph model, in contrast, provides advantages in scalable graph analytical tasks, such as graph matching, path analysis, and graph traversal. RDF-star extends RDF and allows capturing metadata as a first-class citizen. To tap on the advantages of alternative models, the literature proposes different ways of transforming knowledge graphs between property graphs and RDF. However, most of these approaches cannot provide complete transformations for RDF-star graphs. Hence, this paper provides a step towards transforming RDF-star graphs into property graphs. In particular, we identify different cases to evaluate transformation approaches from RDF-star to property graphs. Specifically, we categorize two classes of transformation approaches and analyze them based on the test cases. The obtained insights will form the foundation for building complete transformation approaches in the future.

==> Discussion-draft.tex <==
\subsection{Object Property Statement}
Case 1 represents an \emph{object property} RDF triple with two RDF resources and a predicate connecting them. Based on our evaluation, the three projects mapped this triple into an edge in the generated property graph. The edge connects two nodes (alice and bob) and has type (meets). The edges in the property graphs in Neosemantics and RDF2PG projects can have a type, and the type represents the predicate of the RDF triple. On the other hand, the triple's predicate represents the edge's label in the property graph of the RDF-star Tools project. The property graphs generated by each project had two nodes corresponding with the two RDF resources in the RDF triple (alice and bob). A high level representation of this property graph is shown in Figure~\ref{fig:objectStatement}.
%\vspace{-0.2cm}
\begin{figure}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/objectStatement.pdf}
%\caption{\textbf{Property graph of Object Property RDF Triples}}
\end{subfigure}%
}
\caption{Property Graph of an Object Property RDF Triple}
\label{fig:objectStatement}
\end{figure}

\begin{figure}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/neo4jcase1.pdf}
\caption{\textbf{Neosemantics}}
\end{subfigure}%
%\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/starToolscase1.pdf}
\caption{\textbf{RDF-star Tools project}}
\end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/pgcase1.pdf}
\caption{\textbf{RDF2PG}}
\end{subfigure}
}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
%\centering
\includegraphics[width=.95\textwidth]{figures/legendcase1.pdf}
%\caption{}
\end{subfigure}

}
\caption{The Property Graphs Resulted from Converting Case 1 for each Transformation Project}
\label{fig:objectStatementResults}
\end{figure}

\ntitle{The} default label for the nodes in Neosemantics and RDF2PG graphs is \emph{Resource} while the RDF-star Tools project distinguishes the type of the node by the \emph{kind} property on the node, and in this case, all nodes had the same kind, \emph{IRI} nodes. 
RDF2PG's property graph defined two types for the edges as \emph{ObjectProperty} or \emph{DatatypeProperty} edges (See Figure~\ref{fig:objectStatementResults} (c)). %This case represents an \emph{ObjectProperty} edge as it connects two IRI resources. The \emph{DatatypeProperty} label represents an edge that connects an IRI with a literal object.
\subsection{Datatype Property Statements}
\ntitle{The} four RDF triples in Case 3.1 are \emph{datatype property} statements for the subject (book) and different literal values ("1963-03-22", 100, 20, 55) that represent the objects in each statement, respectively. For RDF-star tools and RDF2PG projects, each literal object was converted to a node in the property graph. The edges resulting in the property graph connect the node of the subject, (book), with the objects' nodes, and the associated predicates (publish\_date, pages, cover, and index) become the edges' types, respectively. Transforming each triple in the RDF graph to an edge in the property graph is a typical RDF-topology preserving transformation. For this example, the transformation would generate four different edges in the property graph (See Figure~\ref{fig:edgesvsproperty} (b) and (c)). In Neosemantics, the same four triples become properties on the subject node, (book) (See Figure~\ref{fig:edgesvsproperty} (a)). Neosemantics transformation is an example of the PG transformation.
%The same applies to the datatype property RDF statements in \textbf{Case 2.1, Case 6.2, Case 9.2, and Case 10}. The transformation of the RDF graph to PG would likely differ depending on the approach followed for treating datatype property statements. 
\begin{figure}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.92\textwidth]{figures/bookprop.pdf}
\caption{\textbf{Neosemantics Property Graph}}
\end{subfigure}
\begin{subfigure}[b]{.7\textwidth}
\centering
\includegraphics[width=.99\textwidth]{figures/bookedges.pdf}
\caption{\textbf{RDF-star Tools Project Property Graph}}
\end{subfigure}%
}\\
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.7\textwidth}
\centering
\includegraphics[width=.99\textwidth]{figures/rdf2pgcase3.pdf}
\caption{\textbf{RDF2PG Property Graph}}
\end{subfigure}
}
\caption{The Property Graph Resulted from Converting Case 3 for each of Neosemantics, RDF-star Tools Project, and RDF2PG graphs}
\label{fig:edgesvsproperty}
\end{figure}

\ntitle{The} RDF-topology preserving transformation and PG transformation approaches resulted in different property graphs when dealing with the datatype property statements (See Section~\ref{sec:mapping}). The transformation of the RDF graphs in Cases 2.1, 6.2, 9.2, and Case 10.1 to property graphs differ in each project depending on the approach followed for treating datatype property statements. 

\ntitle{In} some scenarios, using PG transformation to the property graph would be challenging to represent datatype property statements (e.g., Case 9). If we consider (Mark) as a node with a property (key = age, value = 25), it would not be easy to define how to represent the part (certainty, 0.5) of the asserted triple. Based on our testing, Neosemantics did not transform this triple completely. On the other hand, the RDF-star tools project considered this triple as an edge in the property graph between the two nodes, (Mark) and (25), and an edge type (age). The part (certainty 0.5) of the asserted triple became property for this edge. Using RDF-topology preserving transformation, as exemplified by the RDF-star tools project, for datatype property statements ensures the mapping of all the datatype property RDF-star statements, especially for the embedded datatype property statements.

%\ntitle{In} some scenarios, PG transformation can not guarantee the conversation of all datatype property statements into property graph. For instance, Case 9 is an RDF-star triple that consists of a metadata (ex:certainty, 0.5) for a datatype property statement (ex:Mark ex:age 28). Treating this nested triple as a datatype property statement in the PG transformation would make it challenging to represent the metadata. If we consider (ex:Mark) as a node with a property (key = ex:age, value = 25), it would be difficult to define how to represent the metadata (certainty, 0.5). Based on our testing, Neosemantics did not transform this triple completely, but the RDF-star tools project considered this triple as an edge in the property graph between the two nodes, (ex:Mark) and (25), and an edge type (ex:age). The metadata (certainty 0.5) became a property for this edge.  
%We are not aware of any PG model that allows properties on properties. 
\subsection{An Edge became a Node}
%\ntitle{In} Cases 2.1-2.4, we started noticing the difference in the conversion styles of the three systems in these cases. 
Case 2 represents an RDF resource that has been a predicate in one triple and a subject in other triples. As an RDF graph, the same RDF resource can be referenced by both triples in the same RDF graph (See Figure~\ref{fig:nodeedge} (a)). For Case 2.2 and 2.3, all the evaluated projects treated each RDF triple separately; the RDF resource representing the predicate (mentor) became an edge connecting the subject and object of the first triple. As a subject in the remaining RDF triples, the same RDF resource (mentor) became a node in the generated property graph. As a result, all the evaluated projects mapped the RDF triples into two different property graphs (See Figure~\ref{fig:nodeedge} (b)). The predicate is mapped to both an edge in a subgraph and a node within another subgraph. %Despite the fact that the predicate is shared between the two RDF triples, the resulting property graph is comprised of two disconnected subgraphs, making it impossible to traverse between the subgraphs. The Object 2 is unreachable from Subject 1.

\begin{figure}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/rdfnodeedge.pdf}
\caption{\textbf{Case 2 RDF Triples}}
\end{subfigure}%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.92\textwidth]{figures/nodeEdge.pdf}
\caption{\textbf{Property Graph}}
\end{subfigure}
}
\caption{Conceptual Visualization of RDF Triples in Case 2 vs. the Graph Representation of the Generated Property Graphs}
\label{fig:nodeedge}
\end{figure}

\ntitle{Although} the predicate is shared between the two RDF triples, the resulting property graph comprises two disconnected subgraphs, making it impossible to traverse between them. For example, to retrieve the RDF predicate (mentor) in the RDF graph, we can use the SPARQL query in Listing~\ref{lst:sparqlcase2} to retrieve all the triples, including it. To query the same predicate in the property graph (e.g., Neosemantics property graph), we may need to write multiple queries (e.g., cypher) to retrieve the different representations of the same RDF resource (See cypher queries in Listing~\ref{lst:sparqlcase2}).

\vspace{0.1cm}
\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL vs Cypher Query for Case 2},
label={lst:sparqlcase2}
]
/* SPARQL: Return the RDF triples in the RDF graph */
PREFIX ex: <http://example.com/>
SELECT ?s ?p ?o WHERE { ?s ?p ?o . }

/* SPARQL: Return the name of (ex:mentor) resource */
SELECT ?o where{ ex:mentor ex:name ?o .}

/* Cypher: Return RDF resource (ex:mentor) if it is an edge (i.e., relation) */
MATCH p=()-[r:mentor]->() RETURN p

/* Cypher: Return RDF resource (ex:mentor) if it is a node with url property */
MATCH (n) where n.uri="http://example.com/mentor" return n

/* Cypher: Return both representations of the RDF resource (ex:mentor) */
MATCH (n) where n.uri="http://example.com/mentor"  return 
DISTINCT "node" AS entity, n.uri  AS uri 
UNION ALL
MATCH p=()-[r:mentor]->() 
RETURN DISTINCT "relationship" 
AS entity, type(r) as uri 

/* Cypher: Return property (name) for the RDF resource (ex:mentor) */
MATCH (n) WHERE EXISTS(n.name) RETURN DISTINCT "node" 
AS entity, n.name AS name 

UNION ALL

MATCH ()-[r]-() WHERE EXISTS(r.name) RETURN DISTINCT "relationship" 
AS entity, r.name AS name 

\end{lstlisting}

%\ntitle{Generally,} the literal objects in RDF triples became properties for node in Neosemantics's property graph. However, for the RDF-star tool project, the literal objects were nodes of \emph{kind} literal. The same applies to RDF2PG because it does not support properties for the nodes. 
% We can also find schema triples in many common datasets, such as DBPedia~\cite{lehmann2015dbpedia}.
%apped to a directed labeled arc connecting the subject and the object nodes of that graph. Although these straightforward mappings work for simple triples at the instance level, challenges may arise where predicates also play the role of the subject in other triples as in Fig. 1. Particularly, in the first triple, the predicate is mapped to a labeled arc connecting the two subject/object nodes of the subgraph G1 representing the first triple. When the predicate from the first triple becomes the subject or the object
%of the second triple, it is mapped to another node of the subgraph G2 representing the second triple. As a result, a predicate is mapped to both a labeled arc in the subgraph G1 and a node within the subgraph G2. Despite the fact that the predicate is shared between the two triples, the resulting graph is comprised of two disconnected subgraphs G1 and G2, making it impossible to traverse between the subgraphs. The Object 2 is unreachable from Subject 1
%There is no special treatment for the RDF terms, such as \emph{rdfs:subPropertyOf}, \emph{rdfs:label} except for \emph{rdf:type}. Neosemantics converts the type into a label for the node. In Case 2.4, \emph{ex:friend} as a subject has type \emph{ex:relation}. 
%The DBpedia project maps Wikipedia infoboxes from 27 different language editions to a single shared ontology consisting of 320 classes and 1,650 properties. The mappings are created via a world-wide crowd-sourcing effort and enable knowledge from the different Wikipedia editions to be combined. 

\subsection{Variations of the RDF-star Representation}
%\ntitle{Case} 8 is an example of a embedded RDF-star triples. Based on the evaluation of Neosemantics and the RDF-star Tools projects, the embedded triple became an edge (likes) between two RDF resources (Mary) and (Matt), and the asserted triple was a property (certainty) on edge. %The edge that connected (Mary) and (Matt) had a type or a label (likes) and a property (certainty). %RDF2PG project does not support the embedded RDF-star triples. 
The Cases 8-13 represent different variations of representing embedded RDF-star triples. Neosemantics ignored the RDF-star triples if the object of the asserted triple is a literal value (Case 9), the object is a embedded triple (Case 10), all components of the RDF-star triple are RDF resources (Cases 11.1 and 11.2), the predicate is "rdf:type" (Cases 12.1 and 12.2), or RDF-star triple is a double embedded triple (Case 13). On the other hand, the RDF-star tools project handled most of these cases by treating literal objects as nodes. Cases 10 and 13 cause an error at the parsing phase of the conversion, but both cases can be implemented straightforwardly with the same logic. RDF2PG project does not support embedded RDF-star triples, so none of these cases was converted to a property graph.

\ntitle{The} generated property graphs often have a different graph structure than the RDF-star graph topology. For instance, to query the asserted triple in Case 8, we may use one SPARQL-star query in the RDF-star graph, whereas we may need to write multiple queries in cypher to retrieve the same element in the property graph (See SPARQL-star and cypher queries in Listing~\ref{lst:sparqlstarcase8}). 

%~\ref{lst:sparqlstarcase9}, \ref{lst:sparqlstarcase11} and \ref{lst:sparqlstarcase14}.
\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL-star and Cypher Query for Case 8},
label={lst:sparqlstarcase8}
]
/* SPARQL: Return the (certainty) of the RDF-star triple in Case 8*/
PREFIX ex: <http://example.com/>
SELECT ?value { <<ex:Mary ex:likes ex:Matt >> ex:certainty ?value }
/*Output: 
| value |
| 0.5   | */

/* Cypher: Return property key (certainty) that represents the outer predicate of RDF-star triple in Case 8 */
MATCH (n) WHERE EXISTS(n.certainty) RETURN DISTINCT "node" as entity, 
n.certainty AS certainty 
UNION ALL 
MATCH ()-[r]-() WHERE EXISTS(r.certainty) RETURN DISTINCT "relationship" 
AS entity, r.certainty AS certainty 
\end{lstlisting}
%/* Cypher: Return the relation (ex:likes) of the embedded RDF-star */
%MATCH p=()-[r:likes]->() RETURN p 
%/* Cypher: Return RDF resources of the RDF-star triple in Case 8 */
%MATCH (n) where n.uri="http://example.com/Mary" return n
%MATCH (n) where n.uri="http://example.com/Matt" return n

\ntitle{The} generated property graphs are often lossy graphs that don't contain all the triples. To retrieve all the triples of the element (Alex) in Case 11.2, SPARQL-star returns two triples, but the cypher query would return only one element that represents (Alex) as a node (See Listing\ref{lst:sparqlstarcase11}). The same applies in Case 14.2; the SPARQL-star query would return two values for (certainty), but the cypher query results in one value only for property key (certainty)(See Listing~\ref{lst:sparqlstarcase14}).
\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL-star and Cypher for Case 9 and 10},
label={lst:sparqlstarcase9}
]
/* SPARQL: Return the object of the asserted triple of the RDF-star triple in Case 9*/
PREFIX ex: <http://example.com/>
SELECT ?o ?value { <<ex:Mark ex:age ?o >>  ex:certainty ?value } }
/*Output: 
| o  | value |
==============
| 28 | 0.5   |
 */
/* SPARQL: Return the asserted triple of the RDF-star triple in Case 10*/

 SELECT ?s ?p { ?s  ?p << ex:mainPage ex:writer ex:alice >>}
/*Output: 
| s               | p         |
===============================
| ex:bobshomepage | ex:source |
------------------------------- 
*/
\end{lstlisting}

% same for case 11.1, 12.1, 12.2, 13, 
\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL-star queries for Case 11.2},
label={lst:sparqlstarcase11}
]
/* SPARQL: Return triples of ex:Alex*/
PREFIX ex: <http://example.com/>  
        SELECT ?s ?p ?o 
WHERE {
  {   ?s ?p ex:Alex . }  
  UNION
  { 
    ex:Alex ?p ?o .   
  }
}
/*Output: 
| s                               | p              | o  |
=========================================================
| << ex:alice ex:friend ex:bob >> | ex:mentionedBy |    |
|                                 | ex:age         | 25 |
--------------------------------------------------------------
 */
 
/* SPARQL: Return all the triples for Case 11.2*/
PREFIX ex: <http://example.com/>
SELECT ?s ?p ?o WHERE { ?s ?p ?o . }
/*Output: 

| s                               | p              | o       |
==============================================================
| ex:Alex                         | ex:age         | 25      |
| << ex:alice ex:friend ex:bob >> | ex:mentionedBy | ex:Alex |
--------------------------------------------------------------
 */

/* Cypher: Return nodes with uri = http://example.com/Alex */
MATCH (n) where n.uri="http://example.com/Alex" return n
/*Output: Return 1 node.
*/
\end{lstlisting}


\begin{comment}
Cases 3-8 are different variations of RDF-star triples. RDF-topology preserving transformation ensures handling these cases and converting them into property graphs. Treating each nested triple as an edge in the property graph allows adding metadata as properties for that edge. For example, in Case 6.1, the subject (ex:mainPage) and object (ex:alice) are nodes and the predicate (ex:writer) is type of the edge connecting them. The IRI predicate (ex:source) and the IRI object (ex:bobshomepage) become the (key, value) property for edge (ex:writer). 
This approach could be followed in all RDF-star triples and ensures their mapping into property graph.
\end{comment}
\subsection{Supporting RDF Syntax and Features}
%The three systems transformed them correctly
In Case 3.1 and 3.2, we evaluated the RDF data types and language tags mapping into property graph. The three projects parsed the data types correctly and provided the required details for conversion. Case 14.1 represents an RDF resource as a subject with multiple literal objects for the same predicate. In Neosemantics, the literal values ("Info\_page", "aau\_page") were converted to properties (a list of strings)~\footnote{\url{https://neo4j.com/docs/cypher-manual/current/syntax/values/\#composite-types}} for the triple's subject (college\_page). On the other hand, Both RDF-star tools and the RDF2PG projects treated the literal objects as nodes of type literal, with XSD schema data type annotation and the predicate (subject) as the edge. %In RDF2PG, the edge was further labeled with \emph{datatype property} as it connects an RDF node with a node of type literal.
In Cases 4-6, we evaluated different RDF model features in these cases, such as RDF lists (case 4), blank nodes (case 5), and named graphs (case 6). The three projects transform the RDF list and blank nodes into property graphs. However, named graphs were processed only by Neosemantics.

\subsection{RDF "type" Statements}
Cases 2.4, 5, and 7 contain RDF triples with type predicates such as "\emph{a}" or "\emph{rdf:type}" predicates. Each RDF-star triple would have an IRI subject, type predicate, and an IRI object that most likely represents a \emph{Class} in the RDF graph. %The RDF-topology preserving transformation treats the subject and the object as nodes in the property graphs, and the \emph{rdf:type} predicate is the edge label or type. 
The two projects RDF-star Tools and RDF2PG treated the subject and the object as nodes in the property graphs, and the \emph{rdf:type} predicate is the edge label or type for converting the triples, for example, Case 7. Both projects generated one edge for each triple, such as (alice) is a node connected to the two nodes (Artist) and (Author) in separate edges. On the other hand, Neosemantics treats the \emph{rdf:type} as labels for nodes which does not fit into any transformation approach. %\ntitle{Even} though this transformation follows the RDF-topology preserving transformation, parsing the type predicates depend on user preference in treating the types and whether or not the RDF graph ensembles data and schema. 
\subsection{Multiple Occurrences of the RDF and RDF-star Triple}
In cases 14.2, 15.1, and 15.2, we evaluated the transformation of the same embedded triples from RDF-star graphs to property graphs. In Case 14.2, the RDF-star graph contains the same embedded triples (<<ex:Mary ex:likes ex:Matt>>) multiple times as subjects in different triples with the same predicate (certainty). The Neosemantics and RDF-star Tools project converted only one instance of the triple, the last pared triple (See Listing~\ref{lst:sparqlstarcase14} for the queries used to check). In Case 15.1, the embedded triple acted as a subject with different predicates; both systems generated a property graph with the two nodes (Mary and Matt) with the edge (likes) but two properties (certainty and source) for that edge. %For Case 15.2, the property graphs for the two projects were identical; the two nodes(Mary and Matt) and the edge (likes) and property (certainty). 
RDF2PG could not convert any of these cases as it does not support RDF-star triples.

\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL-star and Cypher for Case 14.2},
label={lst:sparqlstarcase14}
]

/* SPARQL: Return (certainty) of the RDF-star triple in Case 14.2*/
PREFIX ex: <http://example.com/>
SELECT ?value { <<ex:Mary ex:likes ex:Matt >> ex:certainty ?value }
/*Output: 
| value |
=========
| 1     |
| 0.5   |
---------
*/
 
 /* Cypher return all property keys of (likes) relation*/
 MATCH p=()-[r:likes]->() RETURN keys(r)
 /*Output: 
 ["certainty"]
  */
  
 /* Cypher return all property (certainty) of (likes) relation*/ 
 MATCH (n1:Resource)-[r:likes]-(n2:Resource) return r.certainty 
 /* Output:
 0.5
 */
\end{lstlisting}

%\ntitle{In} Case 15, we evaluated the uniqueness of the RDF-star triples in the generated property graphs. This case probably is for evaluating the transformation from the property graph to the RDF graph. However, the duplicate triples were treated differently in the three systems. In the RDF2PG project, all triples were converted into the property graph. However, only one triple was converted in neosemantics and RDF-star tools project, and the redundant triples were ignored. 


\ntitle{From} \textcolor{blue}{our experiments, we conclude that none of the three system's approaches is the best approach that can convert all the cases into property graphs without information loss: Neosemantics fails to transform cases 9, 10, 11.1, 12.1, 12.2, and 13 to property graphs. It also produces partial transformation for cases 11.2 and 14.2. The RDF-star Tools project fails to handle cases 10 and case 13. RDF2PG project fails to convert all the RDF-star cases (Case 8-13). In addition to Cases 6, 14.2, 15.1, and 15.2.}

\ntitle{In} \textcolor{blue}{these experiments, we analyze each system's transformation approach to transform different RDF and RDF-star graphs into property graphs. None of these approaches sticks to one specific transformation approach to convert the test cases and produce a property graph from the RDF and RDF-star graphs. RDF-star Tools project follows the RDF-topology preserving transformation approach, which indicates it creates graph nodes for every subject and object for each RDF triple. However, the RDF-star Tools project converts the predicates and objects of the RDF-star triples into property key and value, respectively. Neosemantics follows the PG transformation in most of the datatype property statements, such as cases 2.1, 3.1, 3.2, 11.2, and 14.1. However, Neosemantics introduces its specific model for handling the types and labels (case 2.4, 5, 6, 7).
RDF2PG project follows the RDF-topology preserving transformation in all the cases, but it introduced new edge labels: ObjectProperty and  DatatypeProperty.
Moreover, the three systems follow the RDF-topology transformation approach for converting case 4, the RDF lists.}


\begin{comment}

\subsection{Datatype Property Statements VS. Object Property Statements}
To better illustrate the difference between the two transformation approaches, consider \textbf{Case 9.1}.  The four RDF triples are \emph{datatype property} statements for the subject \emph{ex:book} and different literal values ("1963-03-22", 100, 20, 55) that represent the objects in each statement, respectively. To convert these triples using an RDF-topology preserving transformation, we convert each of these literal objects to nodes in the property graph. Therefore, the edges in property graph connect the node of the subject, \emph{ex:book}, with the objects' nodes, and the associated predicates (publish\_date, pages, cover, and index) become the edges' types, respectively (See Figure~\ref{fig:twoTypesofMapping}). Generally, we transform each triple as an edge in the property graph. This would generate four different edges in the property graph, the same output we obtain using the transformation of RDF-star tools and RDF2PG projects. In Neosemantics, the same four triples become properties on the subject node, \emph{ex:book}. This transformation is an example of the property graph transformation.

The RDF-topology preserving transformation and PG transformation approaches will result in different property graphs when dealing with the datatype property statements. The transformation of the RDF graphs in Case 2.1, Case 6.2, Case 9.2, and Case 10  would likely differ depending on the approach followed for treating datatype property statements. 
\\
The PG transformation cannot convert all datatype property statements in some scenarios. For instance, Case 4 is an RDF-star triple that consists of a metadata "certainty 0.5" for a datatype property statement "ex:Mark ex:age 28". Treating this nested triple as a datatype property statement in the PG transformation would make it challenging to represent the metadata. If we consider \emph{ex:Mark} as a node with a property \emph{(key = ex:age, value = 25)}, it would be difficult to define how to represent the metadata "certainty 0.5". We are not aware of any property graph model that allows properties on properties. Based on our testing, Neosemantics has ignored this triple completely, but the RDF-star tools project preserves the RDF-star graph. It considers this triple as an edge in property graph between the two nodes, \emph{ex:Mark} and \emph{25}, and an edge type "\emph{ex:age}". The metadata "certainty 0.5" becomes a property for that edge.  
\\
Using RDF-topology preserving transformation for datatype property statements ensures the mapping of all the datatype property RDF statements, especially for RDF-star datatype property statements.
\end{comment}
\begin{comment}

\subsection{Dealing with Complex RDF-star Triples}
Cases 3-8 are different variations of RDF-star triples. RDF-topology preserving transformation ensures handling these cases and converting them into property graphs. Treating each nested triple as an edge in the PG allows adding metadata as properties for that edge. For example, in Case 6.1, the subject \emph{mainPage} and object \emph{ex:alice} are nodes and the predicate \emph{ex:writer} is type of the edge connecting them. The IRI predicate \emph{ex:source} and the IRI object \emph{ex:bobshomepage} become the (key, value) property for edge \emph{ex:writer}. 
This approach could be followed in all RDF-star triples and ensures their mapping into property graph.
\end{comment}

==> Discussion.tex <==
\subsection{Object Property Statement}
Case 1 represents an \emph{object property} RDF triple with two RDF resources and a predicate connecting them. Based on our evaluation, the three projects mapped this triple into an edge in the generated property graph. The edge connects two nodes (alice and bob) and has type (meets). The edges in the property graphs in Neosemantics and RDF2PG projects can have a type, and the type represents the predicate of the RDF triple. On the other hand, the triple's predicate represents the edge's label in the property graph of the RDF-star Tools project. The property graphs generated by each project had two nodes corresponding with the two RDF resources in the RDF triple (alice and bob). A high level representation of this property graph is shown in Figure~\ref{fig:objectStatement}.
%\vspace{-0.2cm}
\begin{figure}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/objectStatement.pdf}
%\caption{\textbf{Property graph of Object Property RDF Triples}}
\end{subfigure}%
}
\caption{Property Graph of an Object Property RDF Triple}
\label{fig:objectStatement}
\end{figure}

\begin{figure}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/neo4jcase1.pdf}
\caption{\textbf{Neosemantics}}
\end{subfigure}%
%\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/starToolscase1.pdf}
\caption{\textbf{RDF-star Tools project}}
\end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/pgcase1.pdf}
\caption{\textbf{RDF2PG}}
\end{subfigure}
}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
%\centering
\includegraphics[width=.95\textwidth]{figures/legendcase1.pdf}
%\caption{}
\end{subfigure}

}
\caption{The Property Graphs Resulted from Converting Case 1 for each Transformation Project}
\label{fig:objectStatementResults}
\end{figure}

\ntitle{The} default label for the nodes in Neosemantics and RDF2PG graphs is \emph{Resource} while the RDF-star Tools project distinguishes the type of the node by the \emph{kind} property on the node, and in this case, all nodes had the same kind, \emph{IRI} nodes. 
RDF2PG's property graph defined two types for the edges as \emph{ObjectProperty} or \emph{DatatypeProperty} edges (See Figure~\ref{fig:objectStatementResults} (c)). 
\subsection{Datatype Property Statements}
\ntitle{The} four RDF triples in Case 3.1 are \emph{datatype property} statements for the subject (book) and different literal values ("1963-03-22", 100, 20, 55) that represent the objects in each statement, respectively. For RDF-star tools and RDF2PG projects, each literal object was converted to a node in the property graph. The edges resulting in the property graph connect the node of the subject, (book), with the objects' nodes, and the associated predicates (publish\_date, pages, cover, and index) become the edges' types, respectively. The transformation would generate four different edges in the property graph (See Figure~\ref{fig:edgesvsproperty} (b) and (c)). In Neosemantics, the same four triples become properties on the subject node, (book) (See Figure~\ref{fig:edgesvsproperty} (a)). Overall, the transformation of the RDF graphs in Cases 2.1, 6.2, 9.2, and Case 10.1 to property graphs differ in each project depending on the approach followed for treating datatype property statements. %Neosemantics transformation is an example of the PG transformation.
%The same applies to the datatype property RDF statements in \textbf{Case 2.1, Case 6.2, Case 9.2, and Case 10}. The transformation of the RDF graph to PG would likely differ depending on the approach followed for treating datatype property statements. 
%Transforming each triple in the RDF graph to an edge in the property graph is a typical RDF-topology preserving transformation. For this example,
\begin{figure}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.92\textwidth]{figures/bookprop.pdf}
\caption{\textbf{Neosemantics Property Graph}}
\end{subfigure}
\begin{subfigure}[b]{.7\textwidth}
\centering
\includegraphics[width=.99\textwidth]{figures/bookedges.pdf}
\caption{\textbf{RDF-star Tools Project Property Graph}}
\end{subfigure}%
}\\
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.7\textwidth}
\centering
\includegraphics[width=.99\textwidth]{figures/rdf2pgcase3.pdf}
\caption{\textbf{RDF2PG Property Graph}}
\end{subfigure}
}
\caption{The Property Graph Resulted from Converting Case 3 for each of Neosemantics, RDF-star Tools Project, and RDF2PG graphs}
\label{fig:edgesvsproperty1}
\end{figure}

%%\ntitle{The} RDF-topology preserving transformation and PG transformation approaches resulted in different property graphs when dealing with the datatype property statements (See Section~\ref{sec:mapping}). The transformation of the RDF graphs in Cases 2.1, 6.2, 9.2, and Case 10.1 to property graphs differ in each project depending on the approach followed for treating datatype property statements. 

\ntitle{In} some scenarios, it would be challenging to represent datatype property statements (e.g., Case 9) in a property graph. If we consider (Mark) as a node with a property (key = age, value = 25), it would not be easy to define how to represent the part (certainty, 0.5) of the asserted triple. Based on our testing, Neosemantics did not transform this triple completely. On the other hand, the RDF-star tools project considered this triple as an edge in the property graph between the two nodes, (Mark) and (25), and an edge type (age). The part (certainty 0.5) of the asserted triple became property for this edge. %% note: Using RDF-topology preserving transformation, as exemplified by the RDF-star tools project, for datatype property statements ensures the mapping of all the datatype property RDF-star statements, especially for the embedded datatype property statements.

\subsection{An Edge became a Node}
%\ntitle{In} Cases 2.1-2.4, we started noticing the difference in the conversion styles of the three systems in these cases. 
Case 2 represents an RDF resource that has been a predicate in one triple and a subject in other triples. As an RDF graph, the same RDF resource can be referenced by both triples in the same RDF graph (See Figure~\ref{fig:nodeedge} (a)). For Case 2.2 and 2.3, all the evaluated projects treated each RDF triple separately; the RDF resource representing the predicate (mentor) became an edge connecting the subject and object of the first triple. As a subject in the remaining RDF triples, the same RDF resource (mentor) became a node in the generated property graph. As a result, all the evaluated projects mapped the RDF triples into two different property graphs (See Figure~\ref{fig:nodeedge} (b)). The predicate is mapped to both an edge in a subgraph and a node within another subgraph. %Despite the fact that the predicate is shared between the two RDF triples, the resulting property graph is comprised of two disconnected subgraphs, making it impossible to traverse between the subgraphs. The Object 2 is unreachable from Subject 1.

\begin{figure}
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/rdfnodeedge.pdf}
\caption{\textbf{Case 2 RDF Triples}}
\end{subfigure}%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.92\textwidth]{figures/nodeEdge.pdf}
\caption{\textbf{Property Graph}}
\end{subfigure}
}
\caption{Conceptual Visualization of RDF Triples in Case 2 vs. the Graph Representation of the Generated Property Graphs}
\label{fig:nodeedge}
\end{figure}

\ntitle{Although} the predicate is shared between the two RDF triples, the resulting property graph comprises two disconnected subgraphs, making it impossible to traverse between them. For example, to retrieve the RDF predicate (mentor) in the RDF graph, we can use the SPARQL query in Listing~\ref{lst:sparqlcase2} to retrieve all the triples, including it. To query the same predicate in the property graph (e.g., Neosemantics property graph), we may need to write multiple queries (e.g., cypher) to retrieve the different representations of the same RDF resource (See cypher queries in Listing~\ref{lst:sparqlcase2}).

\vspace{0.1cm}
\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL vs Cypher Query for Case 2},
label={lst:sparqlcase2}
]
/* SPARQL: Return the RDF triples in the RDF graph */
PREFIX ex: <http://example.com/>
SELECT ?s ?p ?o WHERE { ?s ?p ?o . }

/* SPARQL: Return the name of (ex:mentor) resource */
SELECT ?o where{ ex:mentor ex:name ?o .}

/* Cypher: Return RDF resource (ex:mentor) if it is an edge (i.e., relation) */
MATCH p=()-[r:mentor]->() RETURN p

/* Cypher: Return RDF resource (ex:mentor) if it is a node with url property */
MATCH (n) where n.uri="http://example.com/mentor" return n

/* Cypher: Return both representations of the RDF resource (ex:mentor) */
MATCH (n) where n.uri="http://example.com/mentor"  return 
DISTINCT "node" AS entity, n.uri  AS uri 
UNION ALL
MATCH p=()-[r:mentor]->() 
RETURN DISTINCT "relationship" 
AS entity, type(r) as uri 

/* Cypher: Return property (name) for the RDF resource (ex:mentor) */
MATCH (n) WHERE EXISTS(n.name) RETURN DISTINCT "node" 
AS entity, n.name AS name 

UNION ALL

MATCH ()-[r]-() WHERE EXISTS(r.name) RETURN DISTINCT "relationship" 
AS entity, r.name AS name 

\end{lstlisting}

%\ntitle{Generally,} the literal objects in RDF triples became properties for node in Neosemantics's property graph. However, for the RDF-star tool project, the literal objects were nodes of \emph{kind} literal. The same applies to RDF2PG because it does not support properties for the nodes. 
% We can also find schema triples in many common datasets, such as DBPedia~\cite{lehmann2015dbpedia}.
%apped to a directed labeled arc connecting the subject and the object nodes of that graph. Although these straightforward mappings work for simple triples at the instance level, challenges may arise where predicates also play the role of the subject in other triples as in Fig. 1. Particularly, in the first triple, the predicate is mapped to a labeled arc connecting the two subject/object nodes of the subgraph G1 representing the first triple. When the predicate from the first triple becomes the subject or the object
%of the second triple, it is mapped to another node of the subgraph G2 representing the second triple. As a result, a predicate is mapped to both a labeled arc in the subgraph G1 and a node within the subgraph G2. Despite the fact that the predicate is shared between the two triples, the resulting graph is comprised of two disconnected subgraphs G1 and G2, making it impossible to traverse between the subgraphs. The Object 2 is unreachable from Subject 1
%There is no special treatment for the RDF terms, such as \emph{rdfs:subPropertyOf}, \emph{rdfs:label} except for \emph{rdf:type}. Neosemantics converts the type into a label for the node. In Case 2.4, \emph{ex:friend} as a subject has type \emph{ex:relation}. 
%The DBpedia project maps Wikipedia infoboxes from 27 different language editions to a single shared ontology consisting of 320 classes and 1,650 properties. The mappings are created via a world-wide crowd-sourcing effort and enable knowledge from the different Wikipedia editions to be combined. 

\subsection{Variations of the RDF-star Representation}
%\ntitle{Case} 8 is an example of a embedded RDF-star triples. Based on the evaluation of Neosemantics and the RDF-star Tools projects, the embedded triple became an edge (likes) between two RDF resources (Mary) and (Matt), and the asserted triple was a property (certainty) on edge. %The edge that connected (Mary) and (Matt) had a type or a label (likes) and a property (certainty). %RDF2PG project does not support the embedded RDF-star triples. 
The Cases 8-13 represent different variations of representing embedded RDF-star triples. Neosemantics ignored the RDF-star triples if the object of the asserted triple is a literal value (Case 9), the object is a embedded triple (Case 10), all elements of the RDF-star triple are RDF resources (Cases 11.1 and 11.2), the predicate is "rdf:type" (Cases 12.1 and 12.2), or RDF-star triple is a double embedded triple (Case 13). On the other hand, the RDF-star tools project handled most of these cases by treating literal objects as nodes. Cases 10 and 13 cause an error at the reading phase of the conversion, but both cases can be implemented straightforwardly with the same logic. RDF2PG project does not support embedded RDF-star triples, so none of these cases was converted to a property graph.

\ntitle{The} generated property graphs often have a different graph structure than the RDF-star graph topology. For instance, to query the asserted triple in Case 8, we may use one SPARQL-star query in the RDF-star graph. In contrast, we may need to write multiple queries in cypher to retrieve the same element in the associated property graph (See SPARQL-star and cypher queries in Listing~\ref{lst:sparqlstarcase8}). 
%~\ref{lst:sparqlstarcase9}, \ref{lst:sparqlstarcase11} and \ref{lst:sparqlstarcase14}.
\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL-star and Cypher Query for Case 8},
label={lst:sparqlstarcase8}
]
/* SPARQL: Return the (certainty) of the RDF-star triple in Case 8*/
PREFIX ex: <http://example.com/>
SELECT ?value { <<ex:Mary ex:likes ex:Matt >> ex:certainty ?value }
/*Output: 
| value |
| 0.5   | */

/* Cypher: Return property key (certainty) that represents the outer predicate of RDF-star triple in Case 8 */
MATCH (n) WHERE EXISTS(n.certainty) RETURN DISTINCT "node" as entity, 
n.certainty AS certainty 
UNION ALL 
MATCH ()-[r]-() WHERE EXISTS(r.certainty) RETURN DISTINCT "relationship" 
AS entity, r.certainty AS certainty 
\end{lstlisting}
%/* Cypher: Return the relation (ex:likes) of the embedded RDF-star */
%MATCH p=()-[r:likes]->() RETURN p 
%/* Cypher: Return RDF resources of the RDF-star triple in Case 8 */
%MATCH (n) where n.uri="http://example.com/Mary" return n
%MATCH (n) where n.uri="http://example.com/Matt" return n

\ntitle{The} generated property graphs are often lossy graphs that don't contain all the triples. To retrieve all the triples of the element (Alex) in Case 11.2, SPARQL-star returns two triples, but the cypher query would return only one element that represents (Alex) as a node (See Listing\ref{lst:sparqlstarcase11}). The same applies in Case 14.2; the SPARQL-star query would return two values for (certainty), but the cypher query results in one value only for property key (certainty)(See Listing~\ref{lst:sparqlstarcase14}).
\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL-star and Cypher for Case 9 and 10},
label={lst:sparqlstarcase9}
]
/* SPARQL: Return the object of the asserted triple of the RDF-star triple in Case 9*/
PREFIX ex: <http://example.com/>
SELECT ?o ?value { <<ex:Mark ex:age ?o >>  ex:certainty ?value } }
/*Output: 
| o  | value |
==============
| 28 | 0.5   |
 */
/* SPARQL: Return the asserted triple of the RDF-star triple in Case 10*/

 SELECT ?s ?p { ?s  ?p << ex:mainPage ex:writer ex:alice >>}
/*Output: 
| s               | p         |
===============================
| ex:bobshomepage | ex:source |
------------------------------- 
*/
\end{lstlisting}

% same for case 11.1, 12.1, 12.2, 13, 
\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL-star queries for Case 11.2},
label={lst:sparqlstarcase11}
]
/* SPARQL: Return triples of ex:Alex*/
PREFIX ex: <http://example.com/>  
        SELECT ?s ?p ?o 
WHERE {
  {   ?s ?p ex:Alex . }  
  UNION
  { 
    ex:Alex ?p ?o .   
  }
}
/*Output: 
| s                               | p              | o  |
=========================================================
| << ex:alice ex:friend ex:bob >> | ex:mentionedBy |    |
|                                 | ex:age         | 25 |
--------------------------------------------------------------
 */
 
/* SPARQL: Return all the triples for Case 11.2*/
PREFIX ex: <http://example.com/>
SELECT ?s ?p ?o WHERE { ?s ?p ?o . }
/*Output: 

| s                               | p              | o       |
==============================================================
| ex:Alex                         | ex:age         | 25      |
| << ex:alice ex:friend ex:bob >> | ex:mentionedBy | ex:Alex |
--------------------------------------------------------------
 */

/* Cypher: Return nodes with uri = http://example.com/Alex */
MATCH (n) where n.uri="http://example.com/Alex" return n
/*Output: Return 1 node.
*/
\end{lstlisting}

\subsection{RDF Syntax and Features}
%The three systems transformed them correctly
In Case 3.1 and 3.2, we evaluated the RDF data types and language tags mapping into property graph. The three projects parsed the data types correctly and provided the required details for conversion. Case 14.1 represents an RDF resource as a subject with multiple literal objects for the same predicate. In Neosemantics, the literal values ("Info\_page", "aau\_page") were converted to properties (a list of strings)~\footnote{\url{https://neo4j.com/docs/cypher-manual/current/syntax/values/\#composite-types}} for the triple's subject (college\_page). On the other hand, Both RDF-star tools and the RDF2PG projects treated the literal objects as nodes of type literal, with XSD schema data type annotation and the predicate (subject) as the edge. %In RDF2PG, the edge was further labeled with \emph{datatype property} as it connects an RDF node with a node of type literal.
In Cases 4-6, we evaluated different RDF model features in these cases, such as RDF lists (case 4), blank nodes (case 5), and named graphs (case 6). The three projects transform the RDF list and blank nodes into property graphs. However, named graphs were processed only by Neosemantics.

\subsection{RDF "type" Statements}
Cases 2.4, 5, and 7 contain RDF triples with type predicates such as "\emph{a}" or "\emph{rdf:type}" predicates. Each RDF-star triple would have an IRI subject, type predicate, and an IRI object that most likely represents a \emph{Class} in the RDF graph. %The RDF-topology preserving transformation treats the subject and the object as nodes in the property graphs, and the \emph{rdf:type} predicate is the edge label or type. 
The two projects RDF-star Tools and RDF2PG treated the subject and the object as nodes in the property graphs, and the \emph{rdf:type} predicate is the edge label or type for converting the triples, for example, Case 7. Both projects generated one edge for each triple, such as (alice) is a node connected to the two nodes (Artist) and (Author) in separate edges. On the other hand, Neosemantics treats the \emph{rdf:type} as labels for nodes.% which does not fit into any transformation approach. %\ntitle{Even} though this transformation follows the RDF-topology preserving transformation, parsing the type predicates depend on user preference in treating the types and whether or not the RDF graph ensembles data and schema. 
\subsection{Multiple Occurrences of the RDF and RDF-star Triple}
In cases 14.2, 15.1, and 15.2, we evaluated the transformation of the same embedded triples from RDF-star graphs to property graphs. In Case 14.2, the RDF-star graph contains the same embedded triples (<<ex:Mary ex:likes ex:Matt>>) multiple times as subjects in different triples with the same predicate (certainty). The Neosemantics and RDF-star Tools project converted only one instance of the triple, the last pared triple (See Listing~\ref{lst:sparqlstarcase14} for the queries used to check). In Case 15.1, the embedded triple acted as a subject with different predicates; both systems generated a property graph with the two nodes (Mary and Matt) with the edge (likes) but two properties (certainty and source) for that edge. %For Case 15.2, the property graphs for the two projects were identical; the two nodes(Mary and Matt) and the edge (likes) and property (certainty). 
RDF2PG could not convert any of these cases as it does not support RDF-star triples.

\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:, mentor},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={SPARQL-star and Cypher for Case 14.2},
label={lst:sparqlstarcase14}
]

/* SPARQL: Return (certainty) of the RDF-star triple in Case 14.2*/
PREFIX ex: <http://example.com/>
SELECT ?value { <<ex:Mary ex:likes ex:Matt >> ex:certainty ?value }
/*Output: 
| value |
=========
| 1     |
| 0.5   |
---------
*/
 
 /* Cypher return all property keys of (likes) relation*/
 MATCH p=()-[r:likes]->() RETURN keys(r)
 /*Output: 
 ["certainty"]
  */
  
 /* Cypher return all property (certainty) of (likes) relation*/ 
 MATCH (n1:Resource)-[r:likes]-(n2:Resource) return r.certainty 
 /* Output:
 0.5
 */
\end{lstlisting}

%\ntitle{In} Case 15, we evaluated the uniqueness of the RDF-star triples in the generated property graphs. This case probably is for evaluating the transformation from the property graph to the RDF graph. However, the duplicate triples were treated differently in the three systems. In the RDF2PG project, all triples were converted into the property graph. However, only one triple was converted in neosemantics and RDF-star tools project, and the redundant triples were ignored. 


\ntitle{From} our experiments, we conclude that none of the three projects's approaches is the complete approach that can convert all the cases into property graphs without information loss: Neosemantics fails to transform cases 9, 10, 11.1, 12.1, 12.2, and 13 to property graphs. It also produces partial transformation for cases 11.2 and 14.2. The RDF-star Tools project fails to handle cases 10 and 13. RDF2PG project fails to convert all the RDF-star cases (Case 8-13). In addition to Cases 6, 14.2, 15.1, and 15.2. In summary, out of 44 different RDF and RDF-star triples in the 23 test cases, the Neosemantics and RDF-star Tools project converted around 77\% of the triples, whereas the RDF2PG project converted only 52\% of the same triples.

\ntitle{In} these experiments, we analyze each project's transformation approach to transform different RDF and RDF-star graphs into property graphs. We identify two classes of transformation: RDF-Topology preserving transformation and PG transformation, which we explain in detail below. 
\begin{comment}
None of these approaches sticks to one specific transformation approach to convert the test cases and produce a property graph from the RDF and RDF-star graphs. RDF-star Tools project follows the RDF-topology preserving transformation approach, which indicates it creates graph nodes for every subject and object for each RDF triple. However, the RDF-star Tools project converts the predicates and objects of the RDF-star triples into property key and value, respectively. Neosemantics follows the PG transformation in most of the datatype property statements, such as cases 2.1, 3.1, 3.2, 11.2, and 14.1. However, Neosemantics introduces its specific model for handling the types and labels (case 2.4, 5, 6, 7).



\ntitle{In} \textcolor{blue}{these experiments, we analyze each project's transformation approach to transform different RDF and RDF-star graphs into property graphs. None of these approaches sticks to one specific transformation approach to convert the test cases and produce a property graph from the RDF and RDF-star graphs. RDF-star Tools project follows the RDF-topology preserving transformation approach, which indicates it creates graph nodes for every subject and object for each RDF triple. However, the RDF-star Tools project converts the predicates and objects of the RDF-star triples into property key and value, respectively. Neosemantics follows the PG transformation in most of the datatype property statements, such as cases 2.1, 3.1, 3.2, 11.2, and 14.1. However, Neosemantics introduces its specific model for handling the types and labels (case 2.4, 5, 6, 7).
RDF2PG project follows the RDF-topology preserving transformation in all the cases, but it introduced new edge labels: ObjectProperty and  DatatypeProperty.
Moreover, the three systems follow the RDF-topology transformation approach for converting case 4, the RDF lists.}

\end{comment}

==> Introduction.tex <==
% Graph engines for data management and querying.
% Graphs can be represented in two forms. 
% The decision between the two models depend on many factors such as the flexibility of the models, 
%Similar to the Amazon G1 model~\cite{lassila2021graph} and the domain graph model in the millenniumdb~\cite{millenniumdb}
%\begin{comment}

The most popular models for representing knowledge graphs are: RDF~\cite{berners2001semantic} (Resource Description Framework) and property graphs~\cite{rodriguez2010constructions} (PG). 
While RDF represents knowledge graphs as a set of subject-predicate-object triples, property graphs assign key-value style properties to nodes and edges.
%
%Resource Description Framework (RDF) graphs~\cite{berners2001semantic} and Property Graphs (PG)~\cite{rodriguez2010constructions} are two primary forms of graph data representation~\cite{angles2008survey}. The RDF graph is a set of triples; a triple is represented by three elements: \emph{(subject-predicate-object)} which can be represented as a graph in the form of (node-edge-node). Every node and edge in the RDF graph is identified by an Internationalized Resource Identifier (IRI)~\cite{berners2001semantic}. The property graph contains nodes that can encompass detailed information about a subject and edges that denote the relationship between the nodes~\cite{rodriguez2010constructions}. In the property graphs, arbitrary information can be contained in each node and edge in a key-value form. The key-value information (i.e., properties) represents a specific characteristic or metadata information (for a node or an edge).
%
Recently, RDF-star~\cite{hartig2014foundations} has been proposed as an extension of RDF to enable enriching RDF triples with metadata information by embedding triples in subjects or objects of other triples, which allows providing statements about statements and somewhat resembles adding properties to edges in property graphs. 
%Recently, RDF-star~\cite{hartig2014foundations} has been proposed as an extension for the RDF model to enable enriching RDF triples with metadata information. The metadata can be added to the RDF-star graph by embedding triples in the subject or the object of other triples. Embedding triples into another can mimic adding properties for nodes and edges in the property graph model. The RDF-star extension merges the best property graph qualities into the RDF model, which can be leveraged to bridge the gap between the two data models.

RDF-star graphs and the property graphs are not entirely compatible with one another. Although they both describe data through graphs, their underlying models and semantics are different, leading to many data interoperability issues~\cite{angles2019rdf,lassila2021graph}. 
Metadata or edge properties in RDF-star can be modeled as separate nodes or RDF-star triples.
In contrast, edge properties can only be represented as literal key-value pairs in property graphs. 
In general, it is challenging to transform an RDF-star graph fully into a property graph because of the rich expressiveness of the former. 
The heterogeneity between the two models and their frameworks makes it necessary to study their interoperability, i.e., the ability to map one model to another for data exchange and sharing~\cite{angles2019rdf}. 
%Hence, there is a substantial opportunity for further research on the mapping and the transformation between the two models.

%However, transformation between RDF-star and property graphs is essential for achieving interoperability of the different graph models. The mapping between the two models facilitates reusability of systems and tools between frameworks. 
%RDF-star is supported by a rich ecosystem of data management systems and standards, most notably RDF and RDF-star systems such as Stardog, %~\footnote{\url{https://www.stardog.com/}},
%OpenLink’s Virtuoso, %~\footnote{\url{https://virtuoso.openlinksw.com/}},
%Ontotext GraphDB, %~\footnote{\url{https://www.ontotext.com/}},
%AllegroGraph, %~\footnote{\url{https://allegrograph.com/}}, 
%Apache Jena, %~\footnote{\url{https://jena.apache.org/}},
%and more recently, Oxigraph,  %~\footnote{\url{https://github.com/oxigraph}}, 
%but also query standards, such as SPARQL~\cite{SPARQL} and its extension SPARQL-star\footnote{\url{https://w3c.github.io/rdf-star/cg-spec/editors_draft.html\#sparql-star}} as well as RDF Schema, which allows describing classes of RDF resources and RDF properties~\cite{RDFS}. 
%On the other hand, many graph database systems, such as Neo4j, %~\footnote{\url{https://neo4j.com/}},
%TigerGraph, %~\footnote{\url{https://www.tigergraph.com/}},
%JanusGraph,  %~\footnote{\url{https://janusgraph.org/}},
%RedisGraph, %~\footnote{\url{https://redis.io/docs/stack/graph/}},
%and SAP HANA are based on different variations of the property graph model~\cite{angles2018property,angles2012comparison} and different query languages~\cite{GQL,cypher,deutsch2020aggregation}. 

The mapping between the two models is crucial for data exchange, data integration~\cite{Parent2000DatabaseIT} as well as reusability of systems and tools between the frameworks. 
RDF-star, specifically the RDF model, is recognized as a web-native model that supports data exchange and sharing across different sources because of its formal semantics and the universal uniqueness of resources; IRIs identify every element of an RDF triple~\cite{berners2001semantic}. RDF is a common and flexible model for knowledge representation, and that is exemplified by knowledge graphs that cover a broad set of domains, such as DBpedia~\cite{lehmann2015dbpedia}, YAGO~\cite{suchanek2007yago}, Wikidata~\cite{vrandevcic2012wikidata}, and others~\cite{mccallum2000automating}. 
On the other hand, even with the wide spread of property graph engines, property graphs lack many essential features, such as a schema language, a standard query language, standard data serialization formats, etc. %and federation~\cite{lassila2021graph}. 
Achieving interoperability and reliable transformations between the two frameworks will finally enable us to exploit the benefits of both models. 
%Interoperability between the two frameworks will subsume the benefits and the particular characteristics of the two frameworks, and that cannot be achieved without the ability to map and transform graphs data between the two models. 

%, and unambiguous interpretation~\cite{tomaszuk2020rdf}.
%While RDF to property graph mappings have been studied~\cite{angles2020mapping}, the RDF-star mappings have not yet been researched in detail

In light of this situation, analyzing the transformation between RDF-star and property graphs is highly valuable. The transformation of property graphs to RDF-star graphs has been explored recently~\cite{khayatbashi2022converting}, but the transformation from RDF-star to property graph is yet still to explore. The RDF-star transformation to property graph was previously addressed on the basis of predefined transformations~\cite{hartig2014foundations,angles2020mapping}. However, the state-of-the-art does not cover all mapping issues from the RDF-star into the property graph models. And most importantly, the transformation methods between the two models are not curated for user needs or based on application-specific scenarios. %, and it is our focus in this paper. However, the mapping between the two models still needs further research. 
\begin{comment}
\ntitle{In} \textcolor{blue}{light of this situation, analyzing and studying the transformation between RDF-star graphs and property graphs is highly valuable. The RDF-star transformation to property graph was previously addressed on the basis of predefined transformations~\cite{hartig2014foundations,angles2020mapping}. The transformation of property graphs to RDF-star graphs has been explored recently~\cite{khayatbashi2022converting}, but the transformation from RDF-star to property graph is yet still to explore, and it is our focus in this paper.
However, the mapping between the two models still needs further research. The state-of-the-art does not cover all data mapping issues between the RDF-star and the property graph models. %Hence, the transformation from an RDF-star graph to a property graph may result in information loss because of the property graphs' inability to represent all the RDF-star graph triples.In other cases, the transformation techniques fail to generate a property graph optimized for query-intensive analysis. 
And most importantly, these transformation approaches are not curated for user needs or based on application-specific scenarios. }

\ntitle{The} \textcolor{blue}{ transformation between the RDF-star and property graphs is an essential as a foundation for achieving interoperability of the different class graph models. The mapping between the two models facilitates the reusability of systems and tools between the two frameworks~\cite{thakker2021supporting}. RDF-star is supported by a rich ecosystem of data management systems and standards, most notably RDF stores, the standard SPARQL query language~\cite{SPARQL} and the extended version SPARQL-star\footnote{SPARQL-star Query Language: \url{https://w3c.github.io/rdf-star/cg-spec/editors_draft.html\#sparql-star}}, and RDF Schema which allows to describe classes of resources and RDF properties~\cite{RDFS}. On the other hand, many graph database systems such as Neo4j, TigerGraph, JanusGraph, RedisGraph, and SAP HANA are based on different variations of the property graph model~\cite{angles2018property,angles2012comparison} and different query languages~\cite{GQL,cypher,deutsch2020aggregation}.} %a standard query language that is yet in development~\cite{GQL}. %However, the property graphs support salable storage and querying and are more in line with familiar programming models, which is crucial for graph analytic applications~\cite{lassila2021graph}. 

Recently, RDF-star~\cite{hartig2014foundations} has been proposed as an extension for RDF model to enable the metadata annotation of RDF triples. The metadata can be added in the RDF-star graph by embedding triples in the subject or the object of other triples. Embedding triples into another can mimic the properties in the property graph model. The RDF-star extension merges the best property graph qualities into the RDF framework which may be can be leveraged to bridge the gap between the two data models.
%has been RDF-star~\cite{hartig2014foundations} is a proposed extension to the RDF model that The metadata can be added in the RDF-star graph by embedding triples rather than adding extra triples, as in the reification approach~\cite{hartig2014foundations}. The RDF-star extension merges the best property graph qualities into the RDF framework. Specifically, the RDF-star specification extends RDF's conceptual data model, concrete syntaxes, and query language. 

Resource Description Framework (RDF) graphs~\cite{berners2001semantic} and Property Graphs (PG)~\cite{rodriguez2010constructions} are two primary forms of graph data representation~\cite{angles2008survey}. The RDF graph is a set of triples; a triple is represented by three elements: two nodes (subject and object ) connected by an edge (predicate). Every node and edge in the RDF graph is identified by an Internationalized Resource Identifier (IRI)~\cite{berners2001semantic}. The property graph has nodes that can contain detailed information about a subject and edges that denote the relationship between the nodes~\cite{rodriguez2010constructions}. In the property graphs, arbitrary information can be contained in each node and edge in a key-value form. The key-value information (i.e., properties) represents a specific characteristic or metadata information (for a node or an edge).

The RDF triples can represented in the form of (node-edge-node), %here an example%
whereas in the property graphs, arbitrary information can be contained in each node and edge in a key-value form. The key-value information (i.e., properties) represents a specific characteristic (of a node or an edge). The notion of properties allows the property graph to enclose metadata information such as provenance and time-related information within the graph. Metadata information is of increasing importance, especially in heterogeneous graphs from multiple sources, which require high data quality for data traceability, provenance tracing, knowledge fusion, and many other needs~\cite{metadataEvalution}. 

The RDF model introduces many techniques to deal with the metadata issue, including singleton properties, named graphs, and reification that allows edge properties or statements about "reified" triples. As shown by Hartig~\cite{hartig2014foundations}, these techniques have their shortcomings and do not on their own solve the metadata issue, motivating the development of a new solution. RDF-star~\cite{hartig2014foundations} is a proposed extension to the RDF model that enables the metadata annotation of RDF triples more efficiently. The metadata can be added in the RDF-star graph by embedding triples rather than adding extra triples, as in the reification approach~\cite{hartig2014foundations}. The RDF-star extension merges the best property graph qualities into the RDF framework. Specifically, the RDF-star specification extends RDF's conceptual data model, concrete syntaxes, and query language. 

\ntitle{RDF-star} graphs and the property graphs are not entirely compatible with one another. Although they both describe data through graphs, their underlying models and semantics are different, leading to many data interoperability issues~\cite{angles2019rdf,lassila2021graph}. Metadata properties in RDF-star graphs can be represented as other nodes or RDF-star elements in the graph. In contrast, edge properties can only be represented as literal key-value pairs in the property graphs. Therefore, it is challenging to represent an RDF-star graph fully in a property graph because of the rich expressivity of the former. The heterogeneity between the two models and their frameworks makes it necessary to study their interoperability, i.e., the ability to map one model to another for data exchange and sharing~\cite{angles2019rdf}. Hence, there is a substantial opportunity for further research on the mapping between the two models.
%The RDF model introduces the reification technique, allowing edge properties or statements about "reified" triples. 
%including the RDF-star extension~\cite{hartig2014foundations}. 
%The RDF model provides a way to publish data in a standard format with well-defined semantics, enabling information exchange. Furthermore, the RDF model introduces many reification alternatives, allowing edge properties or statements about "reified" triples, including the RDF-star extension~\cite{hartig2014foundations}. The representation of RDF-star triples is often limited in PGs. Additionally, in PGs, it is possible to have multiple edges connect the same pair of nodes, but in an RDF graph, a relation that connects two nodes is considered a unique object~\cite{lassila2021graph}. Hence, there is a substantial opportunity for further research on the compatibility between the two models~\cite{angles2019rdf,metadataEvalution}.
%For both graph models, the nodes represent entities, edges represent relationships between the entities, and the key-value information (i.e., properties) represents a specific characteristic (of an entity or a relationship). However, RDF graphs are designed to represent statements and are best for representing complex metadata and master data. They are often used to represent complex concepts in a domain, or in situations that require rich semantics and inferences on data. 

\ntitle{The} \textcolor{blue}{ transformation between the RDF-star and property graphs is an essential as a foundation for achieving interoperability of the different class graph models. The mapping between the two models facilitates the reusability of systems and tools between the two frameworks~\cite{thakker2021supporting}. RDF-star is supported by a rich ecosystem of data management systems and standards, most notably RDF stores, the standard SPARQL query language~\cite{SPARQL}\footnote{SPARQL-star Query Language: \url{https://w3c.github.io/rdf-star/cg-spec/editors_draft.html\#sparql-star}}, and RDF Schema which allows to describe classes of resources and RDF properties~\cite{RDFS}. On the other hand, property many graph database systems are based on different variations of the property graph model~\cite{angles2018property} and different query languages~\cite{GQL,cypher}. %a standard query language that is yet in development~\cite{GQL}. %However, the property graphs support salable storage and querying and are more in line with familiar programming models, which is crucial for graph analytic applications~\cite{lassila2021graph}. 
The mapping between the two models is crucial for data exchange and integration~\cite{Parent2000DatabaseIT}. The RDF-star model is recognized as a web-native model that supports data exchange and sharing because its formal semantics allows for easy alignment of meaning and structure across sources, universal uniqueness of resources, and unambiguous interpretation~\cite{tomaszuk2020rdf}. Property graphs lack many features that are an absolute must for data management, e.g. schema language, data serialization formats and federation~\cite{lassila2021graph}. The interoperability between the two frameworks will subsume the benefits and the particular characteristics of the two frameworks, and that cannot be achieved without the ability to map and transform graphs data between the two models. 
}


\ntitle{In} \textcolor{blue}{light of this situation, analyzing and studying the transformation between RDF-star and property graphs is highly valuable. While RDF to property graph mappings have been studied~\cite{angles2020mapping}, the RDF-star mappings have not yet been researched in detail. The RDF-star transformation was previously addressed on the basis of predefined transformations~\cite{hartig2014foundations,angles2020mapping}. However, the mapping between the two models still needs further research. The state-of-the-art does not cover all data mapping issues between the RDF-star and the property graph models. Hence, the transformation from an RDF-star graph to a property graph may result in information loss because of the property graphs' inability to represent all the RDF-star graph triples. In other cases, the transformation techniques fail to generate a property graph optimized for query-intensive analysis. And most importantly, these transformation approaches are not curated for user needs or based on application-specific scenarios. The transformation of property graphs to RDF-star graphs has been explored recently~\cite{khayatbashi2022converting}, but the transformation from RDF-star to property graph is yet still to explore, and it is our focus in this paper.}


\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=-0.0\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={An example RDF-star graph in Turtle star format},
label={lst:motivation}
]
@prefix ex: <http://example.org/> .

<<ex:Alice ex:friend ex:Bob>> ex:mentionedBy ex:Alex .
<<ex:Alex  ex:age   25>>      ex:certainty   0.5 . 
\end{lstlisting}

\begin{figure}[!ht]
\centering
\subfloat[A visual representation of the RDF-star triples in Listing~\ref{lst:motivation}.]
{\qquad \includegraphics[scale=0.5]{figures/rdfstarMotivation.pdf} \qquad }
%\hspace{2cm}
\subfloat[A property graph representing the RDF-star triples in Listing~\ref{lst:motivation}. ] %The property graph has two pieces of information missing that cannot be represented: (ex:mentionedBy, ex:Alex) from the first triple and (ex:certainty, 0.6) from the second triple.
{\qquad  \includegraphics[scale=0.5]{figures/pgMotivation.pdf} \qquad  }
%\hspace{2cm}
%\subfloat[ The property graphs in Figure (a) and (b) could not present the (ex:mentionedBy, ex:Alex) in the second RDF-star triple.]
%{\qquad  \includegraphics[scale=0.5]{figures/Motivation1.pdf} \qquad  }
\caption{A transformation from RDF-star to property graphs in Listing~\ref{lst:motivation}. The strikethrough parts of the triples represent the lost information during the transformation.}
\label{fig:motivationExample}
\end{figure} 
\end{comment}
%<<ex:Alice ex:friend ex:Bob>> ex:mentionedBy ex:Alex .
\begin{comment}

\begin{lstlisting}[
aboveskip=-0.0\baselineskip,
belowskip=0.5\baselineskip,
language=SQL,
breaklines= true,
showspaces=false,
otherkeywords={@prefix, ex:},
keywordstyle=\color{blue},
basicstyle=\ttfamily\scriptsize,
commentstyle=\color{gray},
caption={An example RDF-star graph in Turtle star format},
label={lst:motivation}
]
@prefix ex: <http://example.org/> .

<<ex:Alex ex:age 25>>  ex:certainty 0.5 . 
\end{lstlisting}
\end{comment}
\begin{lstlisting}[
style={st:rdf},
caption={An example RDF-star graph in Turtle star format},
label={lst:motivation}
]
@prefix ex: <http://example.org/> .

<<ex:Alex ex:age 25>>  ex:certainty 0.5 . 

\end{lstlisting}


\begin{figure}[t]
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.4\textwidth}
\centering
\includegraphics[width=.90\textwidth]{figures/rdfstarMotivation.pdf}
\caption{\textbf{RDF-star Graph}}
\end{subfigure}%
\begin{subfigure}[b]{.37\textwidth}
\centering
\includegraphics[width=.90\textwidth]{figures/pgMotivation.pdf}
\caption{\textbf{A property graph}}
\end{subfigure}
}
\caption{Visual Representation of the Transformation of RDF-star triple in Listing~\ref{lst:motivation} into a Property Graph}
\label{fig:motivationExample}
\end{figure}

We illustrate the transformation from RDF-star to property graph through an example. Assume the RDF-star graph consists of the triple in Listing~\ref{lst:motivation} and Figure~\ref{fig:motivationExample}(a) shows a visual representation of this triple. %One way to represent these triples into a property graph is to convert each triple as node-edge-node in the property graph. All Triples' subjects and objects are converted to nodes, such as the mapping of (Alex, 25, Alice, Bob) into nodes as shown in Figure~\ref{fig:motivationExample}(a). This conversion is inspired by the transformation proposed by Hartig~\cite{RDFReconciliation} and based on this proposal, the metadata in the RDF-star triples should be mapped to edge properties in the property graph. For the first triple, the edge (age) is annotated by the metadata (certainty, 0.5). However, the metadata (mentionedBy, Alex) cannot be mapped directly into an edge property because the edges in the property graphs connect only nodes, while representing this metadata requires an edge between a property (mentionedBy) and an existing node in the graph (Alex).
%not edge properties while this metadata  references (Alex), which is an existing node in the graph.
To represent this RDF-star triple in a property graph, one could convert the RDF element (\url{Alex}) into a node in the property graph as shown in Figure~\ref{fig:motivationExample}(b). The triple is converted into a single node (\url{Alex}) with a property \url{(age, 25)}, and based on that, the remining part of the triple \url{(certainty, 0.5)} cannot be represented in this graph. The metadata \url{(certainty, 0.5)} should annotate the property \url{(age, 25)}, but the metadata only describes nodes and edges in the property graph, not other properties. As a result, this transformation from RDF-star to property graph is a lossy transformation that cannot be applied to the given sample RDF-star graph. %Property graphs cannot efficiently represent RDF-star because of the rich expressivity of the latter. 
 
%To represent these RDF-star triples in a property graph, one could convert each triple to nodes and their properties. The RDF elements (Alex, Alice, Bob) can be nodes in the property graph as shown in Figure~\ref{fig:motivationExample}(b).%To represent these RDF-star triples in a property graph, one could convert each triple based on the object's type, an RDF resource, or a literal value. This approach converts the IRI resources (Alex, Alice, Bob) into nodes in the property graph as shown in Figure~\ref{fig:motivationExample}(b). 
%The first triple is converted into two nodes (Alice, Bob) with (friend) as an edge between them. The metadata (mentionedBy, Alex) cannot be mapped directly into an edge property because the edges in the property graphs connect only nodes, while representing this metadata requires an edge between a property (mentionedBy) and an existing node in the graph (Alex). As a result, this transformation from RDF-star to property graph is a lossy transformation that cannot be applied to the given sample RDF-star graph. Property graphs cannot efficiently represent RDF-star because of the rich expressivity of the latter. 
 
%\ntitle{We} evaluate different transformation approaches that map RDF-star graphs to property graphs. We further propose a \emph{hybrid} approach that i) transforms the RDF-star graphs to property graphs, ii) provides the user the ability to select the transformation approach suitable for different application scenarios, and iii) combines two different transformation methods; RDF-topology-preserving transformation and PG transformation.%%%%
%The generated property graph might be incomplete and does not represent all the triples in the original RDF/RDF-star graph. % which is a crutial part
%there is a substantial opportunity for further research.
%in missing the mapping of many triples in the property graphs.  output would ignore
%Some approaches do not provide a complete mapping of RDF/RDF-star graphs to property graphs
%While some system-specific approaches exist, most of them are oriented to format transformation and lack formal foundations and even overall compatibility in some cases~\cite{neosemantics}. Most importantly, these transformation approaches are not curated for user needs or application-specific scenarios.
%\hl{The goal of this paper}

\stitle{Contributions:} In this paper, we make the following contributions:
\begin{inparaenum}[(i)]
     \item We define a set of test cases to experimentally evaluate the mapping approaches that support the transformation from the RDF-star model to the property graph model.
    % \item We identify a set of SPARQL and SPARQL-star queries for the test cases and formulate the associated property graph queries (e.g., cypher query language). We utilize these queries to evaluate the representation of the RDF and RDF-star test cases in the associated property graph model. 
        %\item We identify the shortcomings of state-of-the-art transformation approaches, and we further categorize two classes of transformation: RDF-topology-preserving transformation and PG transformation.
           \item We identify the shortcomings of state-of-the-art transformation approaches, and we further categorize two classes of transformation: RDF-topology-preserving transformation and PG transformation.
        % We utilize these queries to evaluate the property graph model's representation of the RDF and RDF-star test cases.
        % \item We identify a set of SPARQL and SPARQL-star queries for the test cases and formulate the associated property graph queries (e.g., cypher query language) to evaluate the representation of the RDF and RDF-star test cases in the property graph model.
      % \item  We identify the mapping of SPARQL and SPARQL-star queries to the associated property graph queries (e.g., cypher query language) to evaluate the representation of the RDF and RDF-star triples in the property graph model. %test cases to experimentally evaluate the mapping approaches that support the transformation from the RDF-star model to the property graph model.

%\item We propose a user-based transformation model that transforms the RDF-star graphs into property graphs. This model allows the user to combines two approaches for transforming graphs from RDF-star to property graphs; the RDF-topology-preserving transformation and PG transformation.

\end{inparaenum}

The paper is structured as follows: in Section~\ref{sec:preliminaries}, we introduce the relevant background and the formal definitions of both models, RDF-star and property graphs.  
%We also describe different mapping approaches for transforming an RDF-star graph into a property graph. 
In Section~\ref{sec:relatedWork}, we discuss relevant prior work of system-specific approaches for transforming between RDF-star graphs and property graphs. We describe the details of test cases and their examples in Section~\ref{sec:cases}. We present the evaluation of the transformation from RDF-star to property graphs for the state-of-the-art mapping projects in Section~\ref{sec:experiments}. Section~\ref{sec:experiments} also describes different mapping approaches for transforming an RDF-star graph into a property graph and highlights possible scenarios for each approach, %Our proposed hybrid transformation model is described in Section~\ref{sec:approach}, 
 followed by the conclusion in Section~\ref{sec:conclusion}.
%Relevant prior work is described in Section~\ref{sec:relatedWork}

% Although the users can decide the transformation of datatype property statements, the recommended the representation is to have the literal objects as properties on the subject\s nodes. The literal object will not have any outgoing edges that can connect them to other nodes in the graph. 

 




==> approach.tex <==

%Based on our evaluation of the three systems and conversion methods for the test cases, we propose a generic model to convert RDF-star graphs to property graphs. This approach ensures the transformation of all test cases (See Section~\ref{sec:cases}) into property graphs, but it does not ensure the convertibility of the generated property graph back to RDF graphs.\\ 
%We consider the transformation from RDF/RDF-star graphs into property graphs in its core depends on two main approaches: \emph{RDF-topology preserving transformation} %(RDF-TPT)  
%and \emph{property graph transformation}. 
%\subsection{Subject as Predicate or Vice Versa}
%The first triple \emph{ex:book  ex:publish\_date"1963-03-22"$^\wedge$ $^\wedge$xsd:date.} is a datatype property statement. The subject is a 
In practice, the requirements on converting RDF-star (including RDF) to property graphs vary by use case, ontology availability, industry vertical, and performance requirements, however there are recurring patterns of use. These patterns involve the combination of RDF-topology preserving transformation  and PG transformation.

\stitle{Ontology \& Schema Availability} Industries such as financial services, life science, and the military have well-established domain ontologies that can easily be extended to encompass specialized uses cases; however, they often have computationally expensive queries and algorithms that are better suited to property graphs, but they also have data interchange requirements that require the use of the standard domain ontologies. In the latter case, it is useful to convert the ontology using RDF-topology preserving transformations suitable for round-tripping the ontology and converting the RDF graph's data part to property graphs using PG transformation. Another use pattern involves harvesting linked open data for use cases where the property graph is the preferred model. In these cases, the preference is to use the RDF to property graph using the PG transformation approach. The transformation using the PG transformation pattern also makes it easier to include other property graph data and tabular data. In situations where the ontology is essential and the RDF data is highly complex and varied, users may choose to use RDF-topology preserving transformations. Some graph machine learning models also require graphs that model literal property values as vertices.

\stitle{Performance \& Query Complexity} The performance of the queries over graph data depends on the number of edges and nodes the graph contains~\cite{das2014tale}. Therefore, the user may choose to convert the RDF-star graph to a property graph using a specific transformation method to comply with performance requirements. For example, in an application for a smart home, the authors transform the RDF graph into a property graph based on a custom transformation~\cite{baken2020linked}. The authors evaluated the usage of a property graph generated by the custom transformation verse the property graph generated by NSMTX.~\footnote{\url{https://neo4j.com/nsmtx-rdf/}} The property graph of the custom transformation had two nodes and one edge compared to 16 nodes and 15 edges for the property graph generated by the NSMTX plugin. As a result, the execution time for a query to the former graph costs less than the execution time to the NSMTX graph. The custom transformation eliminated many edges (i.e., relations) and converted them into properties.

\begin{algorithm}
\caption{A Generic Transformation Algorithm for Mapping an RDF-star Graph to a Property Graph}
\label{alg:generic}
\begin{scriptsize}
\begin{algorithmic}[1]
\REQUIRE A set of RDF-star Triples $T$
\REQUIRE User Input $i$
\ENSURE A Property Graph $Pg =  (N, E, edge, lbl, P, \sigma)$
\STATE $Pg \leftarrow \emptyset $
\FOR{$t \in T$, such that $t = <s,p,o>$}
 %\IF{$s$ is an embedded triple, such that $s = <\bar{s},\bar{p},\bar{o}>$}
 \STATE{ \quad \tcc{\scriptsize {Check if the triple $t$ is an embedded triple}}}
 \IF{$\bar{t}$ is an embedded triple $\bar{t} = <\bar{s},\bar{p},\bar{o}>$, such that $t = <\bar{t},p,o>$ } 
        \STATE{ \quad \tcc{\scriptsize {Map $\bar{s}$ and $\bar{o}$ into nodes and assign the associated unique identifier for each node based on its type (IRI resource, blank node, or literal value)}}}
         \STATE {$N$ = $N$ $\cup$ \{$\bar{s}$\}}
         \STATE {$lbl(\bar{s})=$ \{"RDF resource"\}}
%         \STATE {add $\bar{s}$ to $N$, 
 %       \\ with $\sigma(\bar{s})= $\{("NodeID", "IRI")\} or $\sigma(\bar{s})= $\{("NodeID", "BlankID")\}  } 
          \STATE {$N$ = $N$ $\cup$ \{$\bar{o}$\}}
 %\STATE {$lbl(\bar{o})=$ \{label\}, such that label $\in$ \{"RDF resource", "Literal"\}}
 \IF{$\bar{o}$ is an RDF resource}
         \STATE {$lbl(\bar{o})=$ \{"RDF resource"\}}
        \ELSE
         \STATE {$lbl(\bar{o})=$ \{"Literal"\}}
         \ENDIF
       %    \STATE {add $\bar{o}$ to $N$,\\ with $\sigma(\bar{o})= $\{("NodeID", "IRI")\} or $\sigma(\bar{o})= $\{("NodeID", "BlankID")\} or
        %   $\sigma(\bar{o})= $\{("NodeID", "ID")\}}
   %   \STATE {add $e$ to $E$}
      \STATE {$E$ = $E$ $\cup$ \{$e$\}}
        \STATE { $edge(e)= (\bar{s},\bar{o}) $}
        \STATE { $lbl(e)= \bar{p} $}
            \STATE  {$pr = $ \{(p, o)\} }
        \STATE {$\sigma(s)=$ pr}
     %   \STATE \colorbox{gray}{ {Algorithm 1 or Algorithm 2}}
    %     \STATE  {add $pr$  to $P$, with $pr = $ \{(p, o)\}}
    %   \STATE  {$\sigma(e)= pr$ }
        \ELSE
         \STATE{ \quad \tcc{\scriptsize {Check if the triple $t$ is a datatype property or an object property triple}}}
        \IF{$o$ is an RDF resource}
        \STATE {$N$ = $N$ $\cup$ \{$s$\}}
         \STATE {$lbl(s)=$ \{"RDF resource"\}}
      %  \STATE {add $s$ to $N$, 
       % \\ with $\sigma(s)= $\{("NodeID", "IRI")\} or $\sigma(s)= $\{("NodeID", "BlankID")\}  }
         \STATE {$N$ = $N$ $\cup$ \{$o$\}}
         \STATE {$lbl(o)=$ \{"RDF resource"\}}
         %  \STATE {add $o$ to $N$,\\ with $\sigma(o)= $\{("NodeID", "IRI")\} or $\sigma(o)= $\{("NodeID", "BlankID")\} }
     % \STATE {add $e$ to $E$}
      \STATE {$E$ = $E$ $\cup$ \{$e$\}}
        \STATE { $edge(e)= (s,o) $}
        \STATE { $lbl(e)= p $}
        
        \ELSE
    %  \STATE{USER INPUT}
       % \Begin{
    %    \Switch{USER INPUT}{
     %      \textbf{when}
\SWITCH {$i$}
\CASE {RDF-Topology Preserving Transformation}
\STATE{ \quad \tcc{\scriptsize {Map $s$ and $o$ into nodes and assign the associated unique identifier for each node based on its type (IRI resource, blank node, or literal value)}}}
     \STATE {$N$ = $N$ $\cup$ \{$s$\}}
         \STATE {$lbl(s)=$ \{"RDF resource"\}}
  %\STATE {add $s$ to $N$, with $\sigma(s)= $\{("NodeID", "IRI")\} or $\sigma(s)= $\{("NodeID", "BlankID")\}  }
  \STATE {$N$ = $N$ $\cup$ \{$o$\}}
   \IF{$o$ is an RDF resource}
         \STATE {$lbl(o)=$ \{"RDF resource"\}}
        \ELSE
         \STATE {$lbl(o)=$ \{"Literal"\}}
         \ENDIF
         %  \STATE {add $o$ to $N$,\\ with $\sigma(o)= $\{("NodeID", "ID")\} } \quad  \tcc{\scriptsize {A unique ID in the graph}}
     % \STATE {add $e$ to $E$}
       \STATE {$E$ = $E$ $\cup$ \{$e$\}}
        \STATE { $edge(e)= (s,o) $}
        \STATE { $lbl(e)= p $}
        
\ENDCASE
\CASE {PG Transformation}
\STATE{ \quad \tcc{\scriptsize {Map only the $s$ into a node and assign the associated unique identifier it based on its type (IRI resource, blank node)}}}
  \STATE {$N$ = $N$ $\cup$ \{$s$\}}
    \STATE {$lbl(s)=$ \{"RDF resource"\}}
 %\STATE {add $s$ to $N$, with $\sigma(s)= $\{("NodeID", "IRI")\} or $\sigma(s)= $\{("NodeID", "BlankID")\}  }
   % \STATE  {add $pr$  to $P$}
     \STATE {$P$ = $P$ $\cup$ \{$pr$\}}
        \STATE  {$pr = $ \{(p, o)\} }
        \STATE {$\sigma(s)=$ pr}
\ENDCASE
\ENDSWITCH
    %}
   % \Switch{$yyy$}{
%\textbf{when} $  0000 | 1111 \quad z:=z$
%\textbf{when}$666$ }
        \ENDIF 
       %  \STATE \HiLi{Transform $t$ following Algorithm 1 or Algorithm 2}
        \ENDIF
    \ENDFOR
     \RETURN $Pg$
\end{algorithmic}
\end{scriptsize}
\end{algorithm}

%Nature of the analytic performed, the frequency of the queries,  
%Additionally, (ii) writing queries to access statement-level metadata is cumbersome because any metadata-related (sub)expression in a query has to be identified by another (sub)expression to match the corresponding metadata triples. Moreover, maintaining metadata and the corresponding querying process in current RDF graph back-end systems remains troublesome~\cite{metadataEvalution}

%In fact, the typical semantic motif query that we need to study agrigenomics-related knowledge networks is a graph pattern representing a chain of given node and relation types, a kind of pattern that is a first-class citizen in Cypher, while the same requires a more verbose syntax in the triple-oriented SPARQL

%One key difference of RDF edge properties compared to edge attributes in property graphs is the fact that the value of an RDF edge property is another node in the graph. In property graphs there is a clear distinction between edges and attributes and attribute values are just strings (or typed primitive values), not things
%\vspace{2cm}
\stitle{Data Sharing.} The transformation approach can be influenced by the users' choice between expressivity verse the meaningful description of the graph data. The RDF-topology preserving transformation allows RDF-star metadata triples (i.e., edge attributes) to be represented as nodes in the property graph, treating them as individual entities. This approach can make the graph representation more expressive for other users to understand and re-use the graph data than the PG transformation approach. The PG transformation can result in many nodes with properties as literal key-value pairs, not explicit edges. This representation can be a natural choice to represent descriptions of nodes, making it a meaningful description of the graph data in specific applications.
%Moreover, RDF-topology preserving transformation may have the capacity to represent complex edge descriptions. The edge properties in property graph can only be represented as literal key-value pairs. In contrast, RDF-star can attach complex descriptions to edges that represent connections to other nodes or literal values. Treating these attributes or properties as separate nodes can help the users to represent complex edge descriptions

%Generic property graph schema applicable for any RDF dataset and can serve many similar domain-independent applications.

%Capacity to represent edge attributes as nodes. As we mentioned above, unlike attributes in LPGs, RDF* edge attributes can be represented as nodes in the graph, allowing them to be treated as individual entities. 2) Better expressivity. RDF* allows every LPG to be efficiently converted into an RDF model. On the other hand, LPGs cannot fully represent RDF* because of the rich expressivity of the latter. 
%3. Arbitrarily complex edge descriptions. With RDF*, graph developers can attach complex descriptions to edges that represent connections to other nodes, literal values (strings), and inter-attribute relationships. In contrast, with LPG, edge properties can only be represented as literal key-value pairs. Publicly sharing graph data by means of well-known data standards.

%\stitle{Graph Storage}
%Conversion cost 
\subsection{Hybrid Approach for RDF-star Transformation}
In what follows, we present an approach for transforming an RDF-star to a property graph that combines the RDF-topology preserving transformation and PG transformation. This approach lets users choose their preferences for converting RDF-star to property graph. The user can decide what transformation approach for the graph. This approach ensures the transformation of the evaluated cases into property graphs, but it does not ensure the convertibility of the generated property graph back to RDF-star graphs.

\ntitle{This} approach (See Algorithm \ref{alg:generic}) converts RDF and RDF-star triples differently. The algorithm follows the RDF-topology preserving approach for converting the RDF-star triples to property graphs. The first step of the algorithm is to check the type of the triple: an RDF-star triple or RDF triple (Line 4).
For the RDF-star triple, the algorithm follows the RDF-topology preserving approach as shown in Line (6-18). The subject and object of the embedded triples are converted to nodes in the results property graphs. The edge type is the embedded triple's predicate. The property key and value of the edges are the asserted triple's predicate and object, respectively.  

\ntitle{For} RDF triples, this approach converts every object property triple into an edge, but it lets the user decide on converting the data property triple. The object property triple connects two RDF resources, and a predicate connects them. The property graph will result in two nodes with the predicate as an edge between them. Line (21 -28) of the Algorithm \ref{alg:generic} summarizes this conversion. 

\ntitle{For} data property triples, the user can input their choice of the transformation approach line (30). The user can follow the RDF-topology preserving transformation line (31 - 43). This transformation will convert the subject and object of the triples into nodes in the property graphs. The algorithm will assign the label (RDF resource) to the subject and one of the labels (RDF resource or Literal) to the object based on its type. Then creates an edge between the subject's node and the object's node. The user may choose PG transformation for converting the data property triples line (44-50). The PG transformation will convert the triple subject into a node with properties created from the predicate and the object of the same triple. The "RDF resource" label labels the subject's node.

\begin{comment}

\begin{enumerate}
    \item RDF Statement Classification:
    \begin{itemize}
        \item Statements will be classified as Object Property or Datatype Property based on the statement object type.
        \item If the statement's object is IRI or Blank node, then it is an Object Property Statement.
        \item If the statement object is literal, it is a Datatype Property Statement.
        \item If the statement is a nested triple, the transformation follows the RDF-topology preserving transformation method regardless of the statement object type.
    \end{itemize}
    \item RDF Statement IRI’s and Blank Nodes Conversion:
    \begin{itemize}
        \item IRI’s and Blank nodes will be converted to nodes.
    \item IRI’s will uniquely identify IRI nodes.
   % \item IRI and Blank node objects should be distinguishable
    \item Node identifier will be derived from IRI or a blank node.
    \end{itemize}
    \item Datatype Property Statement Transformation: Different transformation methods can be followed for the Datatype property statement of non-nested triples. 
\begin{itemize}
   \item RDF-Topology Preserving Transformation or
   \item PG transformation 
   \end{itemize}
\item Object Property Statement Transformation
 \begin{itemize}
 \item Object Property statements will be converted to edges.
\item The edge's source references the statement subject node
\item The edge's target references the statement object node.
\item Edge will be uniquely identified by source, target, and predicate.
     \end{itemize}
\end{enumerate}
RDF-Topology Preserving Transformation and PG Transformation:
\begin{description}[leftmargin=2em,style=nextline]
   \item [RDF-Topology Preserving Transformation] This transformation maps the RDF datatype statements into edges in the PGs. This results in creating nodes of literal values.
    \begin{itemize}
   \item Datatype statements will be converted to edges.
\item The edge's source will reference the statement "subject" node.
\item The edge's target will reference the statement object literal represented as a node.
\item Edge will be uniquely identified by source, target, and predicate.
\item The literal value of the statement object will be represented as a node having properties for value, type, and optional language tag.
    \end{itemize}
   \item [PG Transformation] This Transformation maps the datatype statements to properties on the statement's subject.
    \begin{itemize}
    \item Datatype property triples will be converted to properties.
    \item RDF XSD literal types will be converted to data types depending on the system. 
    \item Multi-valued Datatype property triples will be converted to arrays.

    \end{itemize}
    
\end{description}
\end{comment}


==> experiments_draft.tex <==
This section summarizes the main experiments we perform to evaluate the transformation approaches. Notably, the transformation from RDF and RDF-star to property graphs. The main objectives of this analysis are to 1) identify how different transformation projects map the same RDF and RDF-star triples into property graphs, 2) identify the RDF and RDF-star cases that challenge each transformation project, and 3) identify the transformation approach that each project or tool adopts: (RDF-topology preserving or PG transformation).

\stitle{Transformation projects and their Approaches:} We test the set of cases in Section~\ref{sec:cases} in three different projects that convert RDF and RDF-star graphs to property graphs.
\begin{enumerate}
\item Neosemantics~\cite{neosemantics}: It is a project implemented as a plugin in the Neo4j system. The plugin enables importing RDF-star and its associated vocabularies like (OWL, RDFS, and others) in Neo4j. Neosemantics generally relies on PG Transformation, but with some exceptions that we discuss in detail in this section. For instance, Neosemantics uses the RDF-topology preserving approach to convert RDF lists (Case 4) into property graphs.
 \item RDF-Star Tools Project\footnote{\url{https://github.com/RDFstar/RDFstarTools}}: It is a java project that provides a collection of command-line tools and Java libraries to process RDF-star data and SPARQL-star queries developed by Olaf Hartig~\cite{RDFReconciliation}. This approach mainly adopts RDF-topology preserving transformation for transforming RDF-star graph to property graph.
  \item RDF2PG\footnote{\url{https://github.com/renzoar/rdf2pg.}}: It is A java application to transform RDF databases into property graphs databases~\cite{angles2020mapping}. The project provides different mappings depending on whether or not the input RDF graph has a schema. (i) Schema-dependent: generates a target a property graph schema from the input RDF graph schema and then transforms the RDF graph into a property graph; (ii) schema-independent: creates a generic property graph schema and transforms the RDF graph into a property graph. 
 In this experiment, we evaluate the schema-independent mapping referred to as the \emph{Generic Database Mapping} by the authors. Our analysis aims to evaluate the transformation of the RDF graph to a property graph, not the transformation of the RDF schema to a property graph schema. The schema-independent approach mainly adopts RDF-topology preserving transformation for transforming RDF graph to property graph with some exceptions, such as introducing additional labels for edges in the property graph. 
\end{enumerate}
Table~\ref{tab:mapping} presents the output of mapping different RDF and RDF-star graphs to property graphs in the three project. The transformation output for each project is expressed by our formalization for the property graph model in Section~\ref{sec:preliminaries}. We further analyze the conversion model that each project applies. Each project followed a different class of transformation and produced different property graphs. However, none of the evaluated approaches produces any false mappings such that the information would be represented erroneously. The results mainly differ in the structure of the property graph generated based on test cases or whether the test cases are supported or not. In Table~\ref{tab:mapping}, we use \emph{Not supported} to denote that the project does not consider supporting this case in the research or the implementation.  
We use \emph{Triple is ignored} when the project is claimed to handle the case, but when tested, we found that it skips RDF triples without transforming them to a property graph or producing any exceptional error. \emph{Parsing error} indicates that the system shows an error while reading the graph input.

%\begin{comment}

%%%%%%%%ß  % \small
 % \tiny
\clearpage%
%    \begin{landscape}% Landscape page
 %    \fontsize{7}{11}\selectfont
%% table was here 
% \end{landscape}
 %   \clearpage% Flush page
%\newgeometry{margin=2cm}
\begingroup % restrict scope of reset of \textwidth parameter
%\setlength\textwidth\textwidth %textheight
\setlength{\LTleft}{-4cm}% plus -1fill}
%\setlength{\LTright}{-2cm}%{\LTleft}
\begin{landscape}%
\setlength\tabcolsep{2pt}
 \fontsize{7}{11}\selectfont
%\centering % longtables are centered automatically
\LTXtable{\textwidth}{LongTable} % name of file that contains the table
\end{landscape}

\endgroup
%\restoregeometry
\clearpage

%\end{comment}


==> transformation_approaches.tex <==
\ntitle{The} transformation from RDF-star graphs into property graphs in its core depends on two main approaches: \emph{RDF-topology preserving transformation} and \emph{PG transformation}. The \emph{RDF-topology preserving transformation} is the conversion of an RDF graph while keeping its structure in the generated property graphs. As a generic rule, the RDF-topology preserving transformation transforms each RDF triple into an edge in the generated property graph. The \emph{PG transformation} transforms the RDF graph from a triple-centric into a property-centric graph. PG transformation ensures that RDF triples, mainly in the form \emph{datatype property} triples, are mapped into properties in the nodes of property graphs. In what follows, we explain the difference between the two approaches for RDF and RDF-star triples.
\begin{comment}
\begin{figure*}[th!]
  \centering
  %\includegraphics[scale=0.32]{figures/emblookup_approach.pdf}mulitedges
  \includegraphics[scale=0.6]{figures/Transform.pdf}
  \caption{RDF-topology Preserving Transformation vs. PG Transformation for RDF Triples}
  \label{fig:MappingTypes}
\end{figure*}

\begin{figure*}[th!]
  \centering
  %\includegraphics[scale=0.32]{figures/emblookup_approach.pdf}mulitedges
  \includegraphics[scale=0.6]{figures/Transformstar.pdf}
  \caption{RDF-topology Preserving Transformation VS. PG Transformation - RDF-star Triples}
  \label{fig:MappingTypesstar}
\end{figure*}
\end{comment}
%\vspace{-0.9cm} 

\begin{figure}[t]
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/extriples.pdf}
\caption{\textbf{RDF Triples}}
\end{subfigure}%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/topologyTrans.pdf}
\caption{\textbf{RDF-topology Preserving Transformation}}
\end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/pgtrans.pdf}
\caption{\textbf{PG Transformation}}
\end{subfigure}%
}
\caption{The property graph of the RDF-topology Preserving Transformation (b) VS. property graph of the PG Transformation (c) for the same RDF Triples (a)}
\label{fig:MappingTypes}
\end{figure}
\ntitle{Consider} as an example the set of RDF triples in Figure~\ref{fig:MappingTypes} (a); the triples are \emph{datatype property} triples for the RDF resource (:book).~\footnote{For simplicity, we remove the prefix from the components of the triples in this example.} The RDF-topology preserving transformation approach for converting the RDF triple (:book, :publish\_date, "1963-03-22"$^\wedge$$^\wedge$xsd:date) results into two nodes (book and "1963-03-22") and an edge connecting them (publish\_date). Similarly, the other triples are converted into edges in the property graph (See Figure~\ref{fig:MappingTypes} (b) for the entire graph). Therefore, the output property graph's nodes are RDF resources, blank nodes, and literal values. %The pseudocode of this transformation is explained in the Algorithm\ref{alg:rdfTrdf}. 
%converting these triples into a property graph results in mapping each triple of the RDF graph into an edge in the property graphs. 

\ntitle{On} the other hand, the PG transformation approach converts the same triples into a different property graph topology. This approach distinguishes datatype property triples, and object property triples. The transformation maps every object property triple into an edge; whereas every datatype property triple is converted into a property for the subject of that triple. Unlike the RDF-topology preserving transformation, nodes in the
resulting property graph nodes represent only RDF resources and blank nodes. In the example in Figure~\ref{fig:MappingTypes} (c), the property graph generated by PG transformation consists of only one node representing the RDF resource (:book) associated with a set of properties. The RDF triples' predicates and objects form the properties keys and values, respectively. %(See Figure~\ref{fig:MappingTypes}). %The pseudocode of this transformation is explained in the Algorithm\ref{alg:pgTrdf}.

\begin{comment}

%\subsection{RDF-Topology Preserving Transformation}
\begin{algorithm}
\caption{RDF-topology Preserving Transformation for Mapping an RDF Graph to a Property Graph}
\label{alg:rdfTrdf}
\begin{scriptsize}
\begin{algorithmic}[1]
\REQUIRE A set of RDF Triples $T$ %Given $I$, a set of all IRIs
\ENSURE A Property Graph $Pg =  (N, E, edge, lbl, P, \sigma)$
%\STATE \textbf{Input:} A set of RDF Triples $T$
%\STATE \textbf{Output:} A Property Graph $Pg =  (N, E, edge, lbl, P, \sigma)$
\STATE $Pg \leftarrow \emptyset $
\FOR{$t \in T$, such that $t = <s,p,o>$}
\STATE {$N= N \cup$ \{$s$\} }
% \STATE {add $s$ to $N$, with $\sigma(s)=$ \{("node type", "RDF resource")\} }
 \STATE {$lbl(s)=$ \{"RDF resource"\}}
     \STATE {$N= N$ $\cup$ \{$o$\}}
 \IF{$o$ is an RDF resource}
         \STATE {$lbl(o)=$ \{"RDF resource"\}}
       % \STATE {add $o$ to $N$, with $\sigma(o)=$ \{("node type", "RDF resource")\}  }
        \ELSE
         \STATE {$lbl(o)=$ \{"Literal"\}}
       % \STATE add $o$ to $N$, with $\sigma(o)=$ \{("node type", "Literal")\}  
        \ENDIF
       % \STATE {add $e$ to $E$}
        \STATE {$E= E$ $\cup$ \{$e$\}}
        \STATE { $edge(e)= (s,o) $}
        \STATE {$lbl(e)= p $}
    \ENDFOR
    \RETURN $Pg$
\end{algorithmic}
\end{scriptsize}
\end{algorithm}
 %\vspace{-2cm} 
 \begin{algorithm}
\caption{PG Transformation for Mapping an RDF Graph to a Property Graph}
\label{alg:pgTrdf}
\begin{scriptsize}
\begin{algorithmic}[1]
\REQUIRE A set of RDF Triples $T$
\ENSURE A Property Graph $Pg =  (N, E, edge, lbl, P, \sigma)$
%\STATE \textbf{Input:} A set of RDF Triples $T$
%\STATE \textbf{Output:} A Property Graph $Pg =  (N, E, edge, lbl, P, \sigma)$
\STATE $Pg \leftarrow \emptyset $
\FOR{$t \in T$, such that $t = <s,p,o>$}
\STATE {$N= N$ $\cup$ \{$s$\} }
 \STATE {$lbl(s)=$ \{"RDF resource"\}}
%  \STATE {add $s$ to $N$, with $\sigma(s)=$ \{("node type", "RDF resource")\}  }
 \IF{$o$ is an RDF resource}
     \STATE {$N= N$ $\cup$ \{$o$\}}
    % \STATE {add $o$ to $N$, with $\sigma(o)= $\{("node type", "RDF resource")\}  }
      \STATE {$lbl(o)=$ \{"RDF resource"\}}
      %\STATE {add $e$ to $E$}
       \STATE {$E= E$ $\cup$ \{$e$\}}
        \STATE { $edge(e)= (s,o) $}
        \STATE { $lbl(e)= p $}
        \ELSE
     % \STATE  {add $pr$  to $P$}
       \STATE {$P$= $P$ $\cup$ \{$pr$\}}
        \STATE  {$pr = $ \{(p, o)\} }
        \STATE {$\sigma(s)=$ pr}
 \ENDIF
    \ENDFOR
     \RETURN $Pg$
\end{algorithmic}
\end{scriptsize}
\end{algorithm}

 %%%%%
%\vspace{0.2cm}
\end{comment}
\ntitle{RDF-topology} Preserving transformation and PG transformation are the main approaches commonly adopted to map between the RDF model and the property graph model. There are certain specifications for each approach that can be handled differently, i.e., nodes and edges identifiers and labels. These specifications are implementation details that do not affect the structure of the generated property graph. However, the main challenge for both approaches is mapping an RDF-star graph to a property graph.
\subsubsection{Mapping RDF-star to Property Graphs}
%\ntitle{RDF-star} graph is an RDF graph with embedded triples.
The transformation approaches to map the RDF graph to the property graph can be expected to be the same approaches that convert the RDF-star graph to property graphs. 
In Figure~\ref{fig:MappingTypesstarfail}, we evaluate the two approaches to convert the RDF-star triple (<< :Mary :likes :Matt>> :certainty 0.5) into a property graph. The embedded triple (:Mary :likes :Matt) is mapped to the two nodes (:Mary and :Matt) and the edge (:likes) connecting them in both transformation approaches. The predicate and object of the asserted triple form the edge's property (certainty, 0.5) in the form of a (key, value) pair. %At the very  high level, Algorithm~\ref{alg:rdfTrdfstar} shows the RDF-star transformation to property graphs. In line 4, the mapping of the embedded triple, whether a subject or an object, would be transformed based on the RDF-topology preserving transformation or PG transformation in Algorithm~\ref{alg:rdfTrdf} and Algorithm~\ref{alg:pgTrdf}, respectfully. Similarly, in line 6, the RDF triple could be transformed based on Algorithm~\ref{alg:rdfTrdf} or Algorithm~\ref{alg:pgTrdf}.

\begin{comment}
 \begin{algorithm}
\caption{RDF-topology Preserving Transformation for Mapping RDF-star Graph to a Property Graph}
\label{alg:rdfTrdfstar}
\begin{scriptsize}
\begin{algorithmic}[1]
\REQUIRE A set of RDF-star Triples $T$
\ENSURE A Property Graph $Pg =  (N, E, edge, lbl, P, \sigma)$
\STATE $Pg \leftarrow \emptyset $
\FOR{$t \in T$, such that $t = <s,p,o>$}
 \IF{$s$ is an embedded triple, such that $s = <\bar{s},\bar{p},\bar{o}>$}
        \STATE {add $\bar{s}$ to $N$, with $\sigma(\bar{s})=$ \{("node type", "RDF resource")\}  }
         \IF{$\bar{o}$ is an RDF resource}
         \STATE {Algorithm 1 or Algorithm 2}
        \STATE {add $\bar{o}$ to $N$, with $\sigma(\bar{o})= $\{("node type", "RDF resource")\}  }
         \STATE {add $e$ to $E$}
        \STATE { $edge(e)= (\bar{s},\bar{o}) $}
        \STATE { $lbl(e)= \bar{p} $}
        \ELSE
         \STATE {Algorithm 1 or Algorithm 2}
        \STATE add $\bar{o}$ to $N$, with $\sigma(o)= $\{("node type", "Literal")\}  
        \ENDIF
         \STATE  {add $pr$  to $P$}
        \STATE  {$pr = $ \{(p, o)\} }
       \STATE  {$\sigma(e)= pr$ }
        \ELSE
        \STATE {add $s$ to $N$, with $\sigma(s)=$ \{("node type", "RDF resource")\} } 
 \IF{$o$ is an RDF resource}
        \STATE {add $o$ to $N$, with $\sigma(o)= $\{("node type", "RDF resource")\}  }
        \ELSE
        \STATE add $o$ to $N$, with $\sigma(o)= $ \{("node type", "Literal")\}  
        \ENDIF
        \STATE {add $e$ to $E$}
        \STATE { $edge(e)= (s,o) $}
        \STATE { $lbl(e)= p $}
        \ENDIF
    \ENDFOR
     \RETURN $Pg$
\end{algorithmic}
\end{scriptsize}
\end{algorithm}

\begin{figure*}[th!]
  \centering
  %\includegraphics[scale=0.32]{figures/emblookup_approach.pdf}mulitedges
  \includegraphics[scale=0.6]{figures/rdfstarfail.pdf}
  \caption{RDF-topology Preserving Transformation VS. PG Transformation - Partial Transformation of the RDF-star Triples}
  \label{fig:MappingTypesstarfail}
\end{figure*}
\end{comment}

\begin{figure}[t]
\makebox[\linewidth][c]{%
\begin{subfigure}[b]{.6\textwidth}
\centering
\includegraphics[width=.99\textwidth]{figures/extriplestar.pdf}
\caption{\textbf{RDF-star Triples}}
\end{subfigure}%
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/topologyrdfstar.pdf}
\caption{\textbf{RDF-Topology Preserving Transformation}}
\end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
\centering
\includegraphics[width=.95\textwidth]{figures/pgrdfstar.pdf}
\caption{\textbf{PG Transformation}}
\end{subfigure}%
}
\caption{The PG Transformation (c) property graph cannot represent all the RDF-star triples (a). The property graph of RDF-Topology Preserving Transformation (b) maps them all.}
\label{fig:MappingTypesstarfail}
\end{figure}

\begin{comment}

\begin{algorithm}
\caption{An Transformation Algorithm for Mapping an RDF-star Graph to a Property Graph}
\label{alg:rdfTrdfstar}
\begin{scriptsize}
\begin{algorithmic}[1]
\REQUIRE A set of RDF-star Triples $T$
\ENSURE A Property Graph $Pg =  (N, E, edge, lbl, P, \sigma)$
\STATE $Pg \leftarrow \emptyset $
\FOR{$t \in T$, such that $t = <s,p,o>$}
 %\IF{$s$ is an embedded triple, such that $s = <\bar{s},\bar{p},\bar{o}>$}
 \IF{$\bar{t}$ is an embedded triple, such that $t = <\bar{t},p,o>$ or $t = <s,p,\bar{t}>$}
    %  \STATE {\textcolor{gray}{Algorithm 1 OR Algorithm 2} }
     %    \STATE {add $e$ to $E$}
   %     \STATE { $edge(e)= (\bar{s},\bar{o}) $}
    %    \STATE { $lbl(e)= \bar{p} $}
         \STATE \HiLi { Transform $\bar{t}$ following Algorithm 1 or Algorithm 2}
     %   \STATE \colorbox{gray}{ {Algorithm 1 or Algorithm 2}}
    %     \STATE  {add $pr$  to $P$, with $pr = $ \{(p, o)\}}
    %   \STATE  {$\sigma(e)= pr$ }
        \ELSE
         \STATE \HiLi{Transform $t$ following Algorithm 1 or Algorithm 2}
        \ENDIF
    \ENDFOR
     \RETURN $Pg$
\end{algorithmic}
\end{scriptsize}
\end{algorithm}

\end{comment}

\ntitle{For} both transformation approaches, the asserted triple of the embedded object property triple in the example (<< :Mary :likes :Matt>> :certainty 0.5) is converted into an edge property in the generated property graphs. However, the RDF-star graph may contain asserted triples about embedded data property triples, as in the second RDF-star triple of the example in Figure~\ref{fig:MappingTypesstarfail} (a). The datatype property (ex:Matt ex:age 28) is described by the predicate and object (:certainty, 1), respectively. The transformation of this triple using the PG transformation approach results in the inability to represent the asserted triple in the property graph, whereas the RDF-topology preserving transformation converts all the triples (embedded and asserted triples) into the property graph. The asserted triple of the embedded data property triples could not be transformed using the PG transformation approach because the property graph model does not support properties over other properties. Consequently, the RDF-star graph is converted partially into a property graph by the PG transformation approach without representing the the predicate and object (certainty, 1) (See Figure~\ref{fig:MappingTypesstarfail} (c)).
% The property graph generated using the PG transformation for this example could not represent metadata of this triple, whereas the RDF-topology preserving transformation converts all the triples into the property graph
%\ntitle{Although} the two transformation approaches result in identical property graphs for the RDF-star triples in Figure~\ref{fig:MappingTypesstar}, 
%%% why literal while we know it is no outgoing edges
\ntitle{The} two transformation approaches may result in different property graph models for the same RDF-star graph. % in different cases (See Figure~\ref{fig:MappingTypesstarfail}). 
For some structures of the RDF-star triples, these approaches yield to transform the RDF-star triples into equivalent property graphs. In other scenarios, these two approaches fail to transform the RDF-star graphs into property graphs completely. Moreover, following the same approaches still allows for differences in mapping RDF types, multi-value properties, and other cases. Based on our analysis, none of the evaluated projects sticks to one specific transformation approach to convert the test cases and produce a property graph from the RDF and RDF-star graphs. RDF-star Tools project follows the RDF-topology preserving transformation approach, which indicates it creates graph nodes for every subject and object for each RDF triple. However, the RDF-star Tools project converts the predicates and objects of the RDF-star triples into property key and value, respectively. Neosemantics follows the PG transformation in most of the datatype property statements, such as cases 2.1, 3.1, 3.2, 11.2, and 14.1. However, Neosemantics introduces its specific model for handling the types and labels (case 2.4, 5, 6, 7). Moreover, the RDF2PG project adopted the RDF-topology preserving transformation approach in all cases handled.



%We discuss these scenarios in Section~\ref{sec:experiments}.
%As we will discuss in Section ~\ref{sec:experiments}
\begin{comment}

\section{Property Graph Models in Different Mapping Tools}
\label{sec:PGSmodels}
This section discusses the property graph models in different property graph database systems and tools that work with RDF and RDF-star models.

For all definitions, it is assumed that $\mathfrak{D}$ is a set of data types, in a specific programming language, including a type for strings $S$ and other data types. Each data type $D \in \mathfrak{D}$ has a domain that specify the set of all possible values of type $D$. Let $P$ be the infinite set of all possible properties; that is, a pair $p = (k, v)$ where $k \in dom(S)$ and $v \in \mathfrak{D};$. Let furthermore, Given a set x, $Set(x)$ denote the set of non-empty sets of $x$.

\subsection{RDF-star Tools project}

In this section, we describe the property graph formally as described in~\cite{RDFReconciliation}.  Property Graph can be formalized as follows:
%let $dom(D)$ denote the set of all possible values of type $D$. Given such a set of data types D, the notion of a
\begin{definition} [Property Graph in RDFStar Project~\cite{RDFReconciliation}]

For this definition, it is assumed that $\mathfrak{D}$ is a set of data types, in a specific programming language, including a type for strings $S$ and other data types. Each data type $D \in \mathfrak{D}$, let dom($D$) is the set of all possible values of type $D$. Thus, dom$(S)$ is the set of all strings. Assume that values are unique; that is, for any value $y \in$ dom($D$) of any data type $D \in \mathfrak{D}$, there does not exist another data type $D^{'}\in \mathfrak{D} \backslash $\{$D$\} such that $y \in$ dom$(D^{'})$.
Let $P$ be the infinite set of all possible properties; that is, a pair $p = (k, v)$ where $k \in DM(S)$ and $v \in \mathfrak{D};$. Let furthermore, given a set x, $Set(x)$ denote the set of non-empty sets of $x$. Given a set of data types $\mathfrak{D}$, the property graph can be formalized as follows:

Let $P$ be the infinite set of all possible properties; that is, a pair $p=(k, v)$ where $k \in$ dom $(S)$ and $v \in \bigcup_{D \in \mathfrak{D}}$dom($D$); i.e., $P =$ dom($S$) $\times \bigcup_{D \in \mathfrak{D}}$dom($D$). A \textbf{Property Graph} is a tuple $G = (N, E, src, tgt, lbl_{e}, \alpha) $ such that% $G$ is an edge-labeled directed multigraph with:
\begin{itemize}
    \item $N$: \emph{is a set of nodes},
    \item $E$:  \emph{is a set of edges},
    \item $src$: $E \to N$ \emph{is a function that associates each edge with its source node},
     \item $tgt$: $E \to N$ \emph{is a function that associates each edge with its target node},
    % \item $\rho:E \to(N \times N) $  \emph{is a total function that associates each edge in E with a pair of nodes in N},  
  % \item a function $src : E \rightarrow N $ that associates each edge with its source vertex,
%    \item a function $tgt : E \rightarrow N $ that associates each edge with its target vertex, and
    \item  $lbl_{e}$: $E \rightarrow$ $dom(S)$ \emph{is a function that associates each edge its label; and}
    \item $\alpha$: $(N \cup E) \rightarrow 2^P$\emph{is a function that associates nodes and edges with properties}. % the power set of properties.
   % \item $\sigma$ i
     % \item $\sigma$ is a function $\sigma: (N \cup E) \rightarrow Set(P)$ a partial function that associates a node or edge with a non-empty set of properties.
\end{itemize}
\end{definition}

\subsection{Property Graph in Neo4j Graph Database}
%Multi-value properties RDF triples with literal values are stored in Neo4j as node properties. However, the user had to configure importing the triples with multi-values to store all properties as arrays in Neo4j.
%https://neo4j.com/labs/neosemantics/4.1/import/#handling-multivalued-properties.
%Neo4j~\cite{neo4jDB} is an open-source NoSQL native graph database that utilizes a generic graph structure to store its data. Neo4J stores its data using the property graph model.
%Neo4j's~\cite{neo4jDB} property graph model consists of nodes, relationships (or edges) between them in addition to a set of key-value pairs properties, which further describe them. %CYPHER, a declarative query language similar to SQL but optimized for graphs.
The notion of the Property Graph in Neo4j's~\cite{neo4jDB}  system can be formally described as follow:
\begin{definition} [\emph{Property Graph in Neo4j Graph}]
%For this definition, we assume that $\mathfrak{D}$ is a set of data types, including a type for strings $S$, Let $P$ be the infinite set of all possible properties; that is, a pair $p = (k, v)$ where $k \in dom(S)$ and $v \in \mathfrak{D};$
A \textbf{Property Graph} is a tuple $G = (N, E,P, \rho,lbl_{n},type_{e}, \sigma)$ such that %$G$ is an edge-labeled directed multigraph with:
\begin{itemize}
    \item $N$: \emph{is a set of nodes.} 
    \item $E$: \emph{is a set of edges E that represent the relationships, with} $N \cap E =\phi$
     \item $P$: \emph{ is a finite set of properties,}
    % \item $\rho:E \to(N \times N) $ is a total function that associates each edge in E with a pair of nodes in N,  
   % \item $src$: $E \rightarrow N $ \emph{is a function that associates each edge with its source node,}
    %\item $tgt$: $E \rightarrow N $ \emph{is a function that associates each edge with its target node, and}
    \item $\rho: E \to(N \times N) $: \emph{ is a function that associates each edge with its start and end nodes.}
    \item $lbl_{n}$: $N \rightarrow dom(S)$ \emph{is a partial function that associates nodes with a set of labels.}
    \item $type_{e}$: $E \rightarrow dom(S)$ \emph{is a total function that associates each edge to its type; and}
      \item  $\sigma$: $(N \cup E) \rightarrow Set(P)$ \emph{is a partial function that associates a node or edge with a non-empty set of properties}.
  \end{itemize}  
  \end{definition}
\subsection{Property Graph in RDF2PG Project~\cite{angles2020mapping}}

Assume that $L$ is an infinite set of labels (for nodes, edges, and properties). Nodes and edges cannot have multiple labels. %$V$ is an infinite set of data types. $\mathfrak{D}$ is a finite set of data types. Let furthermore $Set(x)$ denote the set of non-empty sets of $x$.

\begin{definition}[\textbf{Property Graph RDF2PG}]
	 A property graph is defined as a tuple $G = (N, E, P, \rho, \beta, ,\sigma)$, where:
\begin{itemize}
    \item $N$: \emph{a finite set of nodes}. 
    \item $E$: \emph{a finite set of edges.} 
    \item $P$: \emph{a finite set of properties, and $N$, $E$, and $P$ are mutually disjoint sets.}
     \item $\rho:E \to(N \times N) $ \emph{a total function that associates each edge in E with a pair of nodes in N}.  
    %\item a function $src: (E \cup N) \rightarrow L$ that associates each edge with its source node,,
    %\item a function $tgt : E \rightarrow N $ that associates each edge with its target node, and
    \item  $\beta: (E \cup N) \rightarrow L$: \emph{a total function that associates each edge or node with a label.}
  %  \item a function $type_{e} : P  \rightarrow (L \times V)$ is a total function that associates each edge to its type; and
    \item $\sigma: (N \cup E) \rightarrow Set(P)$ \emph{a partial function that associates a node or edge with a non-empty set of properties.}
  \end{itemize}  
  \end{definition}
  
  
\subsection{Canonical Model}
\label{sec:Canonical}
%For this definition, it is assumed that $\mathfrak{D}$ is a set of data types, including a type for strings $S$ and other data types. For each data type $D \in \mathfrak{D}$, let ext($D$) be the set of all possible values of type $D$. Thus, ext$(S)$ is the set of all strings. %Let $P$ be the infinite set of all possible properties; that is, a pair $p=(k, v)$ where $k \in$ ext $(S)$ and $v \in \bigcup_{D \in \mathfrak{D}}$ ext($D$).
%Let furthermore, $\mathcal{P}(x)$ denotes the set of non-empty sets of $x$ for a given set x.
\begin{definition}[\textbf{A Property Graph}]

Given the set of all possible labels $L$, the set of all possible property names $PN$, and the set of all possible property values $D$ including string value $S$, a property graph G is an edge-labeled directed multi-graph such that $G$ = $(N, E, edge, lbl, P, \sigma)$, with:
\begin{itemize}
    \item $N$: \emph{is a set of nodes N}, 
    \item $E$: \emph{is a set of edges E between nodes, with} $N \cap E =\phi$
    \item $edge$: $E \to(N \times N) $ \emph{is a total function that associates each edge in E with a pair of nodes in N, so that if $edge(e_{1}) = (n_{1}, n_{2})$, $e_{1} \in E$ and $ n_{1}, n_{2} \in N $; $n_{1}$ is the source node and $n_{2}$ is the target node.} %An edge $e_{1}$ is a loop if $n_{1}$ = $n_{2}$,}
  % \item \hl{ $lbl$: $ E \rightarrow S$ \emph{is a function that associates each edge with a label.}}
    \item  $lbl$: $(N\cup E) \rightarrow \mathcal{P}($L$)$ \emph{is a function that associates each edge or node with a set of labels.}

   % \item $Pr$: \emph{is an infinite set of all possible properties; that is, a pair} $pr=(k, v)$ where $k \in$ ext$(S)$ and $v \in \bigcup_{D \in \mathfrak{D}}$ ext($D$).
      \item $\sigma$: $(N \cup E) \rightarrow \mathcal{P}(P)$ \emph{is a function that associates a node or edge with a non-empty set of properties $P$ defined as a set of key-value pairs ($k,v$) where $k \in PN$ and $v \in D$}
  \end{itemize}  
  

\end{definition}

%To ensure the model's coverage for all systems' representations, we also consider mapping any possible IRI to a distinct string representing a local name. Given $I$, \emph{a set of all IRIs,} $localName$: $ I \rightarrow S $ \emph{is a function that maps an IRI to a string that represents the local name of an RDF resource.}

To ease all systems' output representation, we also consider mapping any possible IRI to a distinct string representing a local name. Given $I$, a set of all IRIs, $localName$ is a function that maps an IRI to a string that represents the local name of an RDF resource\footnote{In Neo4j, the user can configure the local Name for RDF terms such as subPropertyOf, subClassOf, Class, etc.}. For example, the local name for the RDF resource (http://example.com/meets) $localName$("http://example.com/meets") is "meets". We use this function in the output representation in Section~\ref{sec:experiments}.

\end{comment}
